SLAM for Visually Impaired People: a Survey

In recent decades, several assistive technologies have been developed to improve the ability of blind and visually impaired (BVI) individuals to navigate independently and safely. At the same time, simultaneous localization and mapping (SLAM) techniques have become sufficiently robust and efficient to be adopted in developing these assistive technologies. We present the first systematic literature review of 54 recent studies on SLAM-based solutions for blind and visually impaired people, focusing on literature published from 2017 onward. This review explores various localization and mapping techniques employed in this context. We systematically identified and categorized diverse SLAM approaches and analyzed their localization and mapping techniques, sensor types, computing resources, and machine-learning methods. We discuss the advantages and limitations of these techniques for blind and visually impaired navigation. Moreover, we examine the major challenges described across studies, including practical challenges and considerations that affect usability and adoption. Our analysis also evaluates the effectiveness of these SLAM-based solutions in real-world scenarios and user satisfaction, providing insights into their practical impact on BVI mobility. The insights derived from this review identify critical gaps and opportunities for future research activities, particularly in addressing the challenges presented by dynamic and complex environments. We explain how SLAM technology offers the potential to improve the ability of visually impaired individuals to navigate effectively. Finally, we present future opportunities and challenges in this domain.

==> texs/back-up/bck-03_results.tex <==
%
% Section 3: Result
\section{Result}
\label{results}
In this section, the findings of SLR are presented. Figure \ref{distribution_of_papers} shows the number of studies included in this review, which focused on BVI navigation using SLAM techniques. As shown in the figure, although only papers published in the first half of 2023 are included in this review, they constitute a substantial portion of the total. The growth in the number of studies in this domain suggests an advancement in SLAM techniques and an increase in their usage for developing navigation technologies for visually impaired individuals. 
This section is divided into four parts to answer the research questions. It discusses the types of SLAM techniques used to develop assistive technologies for visually impaired navigation, delves into the advantages and limitations of these techniques, highlights the challenging scenarios addressed, and presents the attributes of the SLAM technology that contribute to the enhancement of visually impaired navigation.

% Figure 5. Publications included in this review on SLAM-based BVI navigation, by year
\begin{figure}[h]
    \centering
    \includegraphics[scale=0.4]{images/05_distribution_of_papers.png}
    \caption{\textbf{Publications included in this review on SLAM-based BVI navigation, by year}}
    \label{distribution_of_papers}
\end{figure}

%
% RQ1
%
\subsection{RQ1. What localization and mapping approaches are used for the navigation of the visually impaired?}
Since there are many different types of SLAMs designed with different types of sensors, for different applications, and for different scenarios, in this section, we focus on reviewing the types of SLAM that have been used for navigation of visually impaired people. It is a key technology in robotics and computer vision and has the potential to assist visually impaired individuals with navigation. This can help visually impaired individuals by providing real-time location information, maps, and spatial awareness. Among the 54 papers surveyed, three strategies were common, as shown in Table \ref{rq1_slam_type}. In this table, we use the exact terms mentioned in the literature for the localization and mapping techniques. 

The majority of studies have leveraged established SLAM techniques, such as ORB-SLAM, while some studies have developed new solutions tailored to their needs. For example, \cite{jin2020combining} proposed visual simultaneous localization and mapping for the moving-person tracking (VSLAMMPT) method. The proposed method was designed to assist people with disabilities, particularly visually impaired individuals, in navigating indoor environments. Additionally, various studies have used the SLAM components of existing frameworks, such as ARCore and ZED camera SLAM.

It is worth noting that several studies have employed VIO and SLAM as the core components in their proposed systems, whereas others have employed them to enhance the robustness of localization \cite{cheng2021hierarchical}, for comparison with alternative localization approaches \cite{lu2021assistive}, or to develop new localization methods \cite{crabb2023lightweight}. For example, \cite{crabb2023lightweight} presented a novel localization approach specifically designed for individuals with visual impairment. This method combines visual landmark identification, VIO, and spatial constraints derived from a two-dimensional (2D) floor plan.

SLAM methodologies can be categorized into feature-based, direct, and optical-flow techniques. Feature-based methods extract and describe feature points in an image, which are then matched across different images for tracking and mapping. On the other hand, direct methods directly calculate the luminosity changes of pixel blocks. Optical flow methods utilize the optical flow changes in feature points, pixel gradient points, or the entire image to track and map the environment \cite{chen2021wearable}.

SLAM algorithms are further categorized into optimization- and filtering-based methods, each with distinct approaches to map creation and agent localization. Optimization-based, often referred to as Graph SLAM, treats the problem as a large optimization task, where the goal is to find the set of poses and landmark positions that best explain the observed sensor measurements. This is typically achieved by constructing a graph in which nodes represent  agent poses or landmarks and edges represent constraints or observations between them. The solution is determined by minimizing the global cost function, which represents the error between the predicted and actual measurements, using nonlinear optimization techniques. On the other hand, filtering-based SLAM uses recursive Bayesian filters, such as the Extended Kalman Filter (EKF) or Particle Filter, to incrementally update the map and the  agent's position as new sensor data arrive.

Systems such as ORB-SLAM and RTAB-Map are feature- and optimization-based, employing features and graph optimization for mapping and localization. Conversely, LSD-SLAM and DSO are examples of direct and optimization-based SLAM. Some systems, such as Semantic SLAM, may adopt either approach, depending on their implementation. It is important to note that the method and type of SLAMs are not directly mentioned in all papers, so the information provided here is a general categorization based on common practices within each category.

The reviewed studies demonstrate the versatility of SLAM in various navigation scenarios. The specific implementation and aspects addressed in each study varied depending on the application. SLAM can be employed in environments that lack a map and can dynamically create it while navigating. This involves simultaneous map creation and localization within an environment. Alternatively, SLAM can be employed to generate maps for subsequent navigation. In this case, SLAM first builds a map of the environment and then the map is utilized during navigation. Studies have also used SLAM odometry for navigational tracking. Odometry provides a continuous estimate of the position and orientation of an agent based on the sensor readings.

% Table 10. RQ1. Localization and mapping approaches used for visually impaired navigation
\input{texs/tables/t10_RQ1_SLAM_type}

Our analysis, underscored by the classifications in Table \ref{rq1_slam_type}, indicates a strong preference for feature-based and optimization-based SLAM approaches for visually impaired navigation. This preference is likely due to the robustness and efficiency of these methods in processing visual data, which is key for real-time assistive navigation. The common use of visual sensors in SLAM techniques can be attributed to advances in computer vision and image processing, which enhance navigation capabilities by providing rich environmental information. This makes visual-sensor-based SLAM techniques the most used in the implementation of assistive technologies for the blind, offering a cost-effective, versatile, and accurate solution for real-time navigation and spatial awareness.

Figure \ref{SLAM_over_time} provides insight into the use of various localization and mapping techniques for visually impaired navigation from 2017 to the date when SLR was conducted (July 2023). This figure illustrates that visual techniques has consistently been used across all years. Although many other techniques also operate based on visual data, we mentioned each of these techniques, as indicated in the referenced studies. 

The utilization of semantic SLAM and Cartographer SLAM signifies a recent trend towards leveraging advanced spatial understanding and mapping capabilities for visually impaired navigation. Semantic SLAM incorporates higher-level scene interpretation and enhances users’ contextual awareness. On the other hand, Cartographer SLAM provides SLAM in 2D and 3D across various platforms and sensor configurations, offering innovative solutions to tackle the diverse challenges associated with BVI navigation.

ORB-SLAM algorithms, including ORB-SLAM (published in 2015), ORB-SLAM2 (published in 2017), and ORB-SLAM3 (published in 2021), have gained popularity because of their robustness and performance. This can be attributed to its efficient feature extraction and matching techniques, making it well suited for real-time navigation applications.

Customized techniques have been developed to meet specific needs. This trend indicates that researchers have adjusted the SLAM techniques to better match the specific requirements of their intended applications. This suggests closer integration of SLAM with domain-specific needs.
 % Fig. 6. Evolution and adoption of SLAM techniques in BVI navigation systems over time.
\begin{figure*}
    \centering
    \includegraphics[scale=.5]{images/06_SLAM_over_time.png}
    \caption{\textbf{Evolution and adoption of localization and mapping techniques in BVI navigation systems over time.}}
    \label{SLAM_over_time}
\end{figure*}

% 
% RQ2
%
\subsection{RQ2. What are the advantages and limitations of SLAM techniques for BVI navigation?}

\subsubsection{Advantages}
Unlike many localization approaches, such as RFID- or GPS-based methods, which require infrastructure setup, SLAM does not depend on pre-existing infrastructure. It operates autonomously by creating maps and understanding the surroundings in real-time.
% , making it highly adaptable to changing environments. 
SLAM relies on data captured by sensors already present on many mobile devices, such as smartphones, and offers a cost-effective solution for accurate localization and mapping without the need for additional hardware or subscription services.

One of the most important advantages of SLAM is its potential for real-time positioning, which determines the agent’s current location and orientation. Systems leveraging ORB-SLAM, for instance, excel in pose estimation by integrating various data types, including visual, inertial, and depth information, thus enhancing accuracy beyond conventional methods \cite{xie2022multi}. This feature is pivotal not only for effective navigation but also for obstacle detection and avoidance, ensuring the safety and confidence of visually impaired users as they navigate through immediate environments \cite{xie2022multi, rui2021multi}.

SLAM's ability to reuse and update maps incrementally allows for a high degree of environmental adaptation. Its capacity to relocalize within prebuilt maps or expand them as necessary ensures that users can rely on updated information for navigation \cite{zhang2019arcore, bai2018virtual}. This adaptability is further enhanced by the capability of the system to handle dynamic environments, making it invaluable for visually impaired users who require real-time path adjustments in response to moving obstacles \cite{jin2020combining, ou2022indoor}.

Detailed environmental mapping facilitated by SLAM, ranging from two-dimensional layouts to complex 3D geometric and semantic maps, provides comprehensive spatial understanding \cite{zhang2023research, slade2021multimodal, liu2020indoor}. Environmental awareness is critical for path planning and collision avoidance. Furthermore, the integration of semantic mapping enriches spatial understanding by adding contextually rich information to maps, thereby facilitating more informed decision-making and interaction with the environment \cite{chen2021wearable, zhao2019multi}.

The integration of different types of sensors and technologies with SLAM significantly expands the scope of its application. By integrating techniques such as object detection algorithms or combining RGB-D and IMU sensor data, SLAM systems achieve a multilayered perception of the environment \cite{xie2022multi, goswami2023efficient}. Sensor fusion enhances a system's ability to detect and classify objects, accurately navigate, and handle dynamic elements within the environment, thereby offering a more holistic assistive solution \cite{hakim2019indoor}.

The cost-effectiveness of SLAM-based solutions attributed to their reliance on widely available low-cost sensors makes this technology particularly interesting. Systems employing monocular cameras or wearable RGB-D cameras exemplify how SLAM can be implemented in a cost-effective manner without compromising functionality, thus making advanced navigational aids accessible to more users \cite{hakim2021indoor, hao2022detect}.
The advantages of SLAM, derived from the literature, are listed in Table~\ref{rq2_advantages}.

\input{texs/tables/t11_RQ2_SLAM_advantages}

\subsubsection{Limitations}
Although SLAM technologies show great potential for improving navigation aids for the visually impaired, they are not without their limitations. These limitations can significantly impact the effectiveness and reliability of SLAM-based assistive systems.

A notable challenge is the computational complexity and the associated demand for system resources. The implementation of advanced SLAM algorithms and the integration of deep learning frameworks for semantic understanding introduce significant computational overhead \cite{li2022sensing, liu2020indoor}. This complexity can compromise the real-time performance, which is crucial for assistive navigation. The need for appropriate hardware to process high-resolution data further underscores this limitation, potentially restricting the deployment of SLAM-based systems \cite{rui2021multi}.

The effectiveness of SLAM is dependent on its environmental characteristics. Accurate mapping and localization depend on the presence of distinct geometric features. In environments lacking such features or dynamically changing settings, SLAM systems may struggle to maintain accurate localization, thereby leading to navigation errors \cite{zhang2017indoor}. This limitation is particularly evident in feature-poor areas such as long corridors or spaces with uniform surfaces, where loss of localization can occur \cite{hou2022knowledge}.

Another critical limitation is the dependence on initial data or pre-existing maps. Some SLAM systems require sighted individuals to pre-map the environment, which can limit the flexibility and immediate usability of unmapped or altered spaces \cite{zhang2019arcore, bai2018virtual}. This reliance on prior mapping can be a significant hurdle for deploying SLAM-based navigation aids in diverse and changing environments \cite{son2022wearable, chen2020navigation}.

Drifting errors present a substantial challenge for maintaining the long-term accuracy of SLAM systems. Over time, small inaccuracies can accumulate, leading to significant deviations from the true trajectory, which can disorient users and compromise the navigation safety \cite{ahmetovic2023sonification}. In addition, the ineffectiveness of some SLAM systems for generating dense navigation maps limits their utility in providing the detailed guidance required for visually impaired navigation, necessitating further algorithmic enhancements \cite{xie2022multi}.

The performance of SLAM in dynamic environments, characterized by moving obstacles and changing conditions, remains a critical concern. Systems may fail to adapt quickly to such changes, leading to potential navigation errors and safety risks for visually impaired users \cite{lu2021assistive}.

Some SLAM applications require external calibration or setup, such as placement of calibration boards in specific environments. This requirement can limit the spontaneity and ease of use of SLAM-based navigation aids because it imposes additional  constraints \cite{lalonde2018localizing}. 
Table \ref{rq2_limitations} outlines the overall limitations of SLAM, derived from the publications under review.

% Table 12. Limitations of SLAM techniques mentioned in the studies included in the SLR.
\input{texs/tables/t12_RQ2_SLAM_limitations}

% 
% RQ3
%
\subsection{RQ3. What challenging situations have been addressed?}
Optimal pathfinding, perception of the surroundings, and obstacle avoidance are crucial for navigation. The precise localization of a visually impaired user within the environment is essential for these functions to operate effectively. Our surveyed papers addressed the localization and mapping problems using various techniques. Some of these studies explored other navigation-related challenges. We categorized these challenges into two groups: those relevant to environmental complexities, and those related to the sensors used to receive environmental data. Dynamic obstacles and crowded spaces constitute the challenges in the first group, whereas challenges related to changing lighting conditions and the rapid motion of users that results in motion blur fall into the second group. Table \ref{rq3_challenges} lists studies that investigated these challenges through the integration of SLAM with other approaches. In the following section, we discuss the studies that address these challenges.


% Table 13. Challenges addressed in reviewed studies using SLAM techniques
\input{texs/tables/t13_RQ3_challenges}


% 4.3.1 Environmental complexities
%
\subsubsection{Environmental complexities}


%
% Crowded scenarios
%
\textbf{Crowded scenarios}
Navigating crowded environments presents significant challenges for the visually impaired, leading to increased collision risks and difficulties in maintaining personal space. The absence of visual information makes it difficult to measure the distance, perceive crowd density, and locate landmarks or places of interest.


Navigation in crowded environments also poses challenges for assistive technology. For example, in assistive systems that operate based on SLAM, the presence of numerous dynamic elements, such as moving individuals and objects, introduces ambiguity into feature detection and tracking, leading to difficulties in accurately estimating the pose of the user and structure of the environment. The dynamic nature of crowds also hinders loop closure detection, disrupts map consistency, and contributes to drifts. Moreover, the lack of distinct visual landmarks in crowded scenes represents a reliable localization challenge that potentially reduces the robustness and accuracy of the overall SLAM system. Addressing these challenges requires the development of new approaches to address the complexity of such environments effectively. Several studies have examined this issue.


\cite{zhang2023research} presented a guide mobile robot engineered for the complexities of navigating different environments while considering dynamic objects and human presence. The robot could handle crowded environments with multiple dynamic objects. To accomplish this, the robot leveraged a spatial risk map, a tool that evaluates potential object-occupied spaces, to chart a path that effectively minimizes disruptions. This paper presents experiments in which a robot successfully guided a user through the passage of multiple objects and people.


In another study, \cite{qiu2022egocentric} introduced an egocentric human trajectory forecasting model designed for navigation in crowded environments. By leveraging a wearable camera, the model captures detailed surroundings and the user's past trajectory to predict their future. The trajectories obtained using ORB-SLAM3 were used to train the egocentric human trajectory forecasting model, which predicted the wearer's future trajectory based on the contextual cues captured by the wearable camera and the wearer's past trajectory.


Additionally, \cite{lu2021assistive} addressed challenges in crowded environments using a combination of SLAM and Ultra-Wideband (UWB) positioning. However, the SLAM algorithm was found to be less effective in environments with dynamic obstacles such as pedestrians. The algorithm finds features of dynamic obstacles moving along with the robot as the assistive device, and thus it was misled that the robot did not move at all. However, using UWB positioning mitigates this issue.


In \cite{kayukawa2020guiding}, the method addressed crowded environments by recognizing and predicting people's behavior while anticipating the collision risk. The system advises users to adjust their walking speed (on-path mode) or to choose alternative routes (off-path mode). This involves comparing the 3D point cloud map to the real-time LiDAR and IMU sensor data. The system then predicts the future position and velocity of the user in order to avoid collisions.

An intelligent autonomous scooter was developed in \cite{mulky2018autonomous} for navigating environments with small safety margins and highly dynamic pedestrian traffic such as sidewalks with numerous obstacles and pedestrians. The authors proposed a hybrid mapping solution that combines far-field and near-field mapping to navigate through dynamic environments. This approach utilizes sensor fusion to adapt dynamically to complex and cluttered environments.

%
% Dynamic objects
%
\textbf{Dynamic objects}
Several publications have not directly addressed the challenge of crowded environments, and have only focused on dealing with the presence of dynamic objects within the scene. In the system proposed by \cite{ou2022indoor}, dynamic objects can be identified, and average depth information can be provided to the user. When a dynamic object belongs to a predefined class such as a person, it can also be tracked between frames in the SLAM pipeline. The system is capable of identifying and tracking dynamic objects after ego-motion estimation to obtain average depth information. Subsequently, it can estimate the poses and speeds of these tracked dynamic objects and relay this information to the users through acoustic feedback. Depth information helps users maintain social distancing in public indoor environments such as shopping malls.
To address the challenge of dynamic objects, \cite{jin2020combining} proposed a new method called visual simultaneous localization and mapping for moving person tracking (VSLAMMPT). This method was designed to handle dynamic environments in which objects constantly move. The system also uses the expected error reduction with active-semi-supervised learning (EER–ASSL)-based person detection to eliminate noisy samples in dynamic environments. This aids in accurate detection and avoidance of dynamic obstacles.

\cite{zhao2019multi} utilized YOLOv3 to detect common objects in a corridor, including people, which were identified as obstacles. The system sends information about obstacles to users every five seconds when the distance between the user and the obstacle is less than 10 meters. For example, it may notify the user, "A person is located 2.8 meters ahead."


%
% 4.3.2 Sensor-related
%
\subsubsection{Sensor-related}


\textbf{Changes in lighting condition}
Lighting changes pose a hurdle to visual SLAM systems. Illumination variations alter the visual features, interfere with accurate detection and matching across frames, impact pose estimation, and map-building robustness. SLAM relies on distinctive features for operation; however, lighting changes introduce ambiguities, noise, and errors, which affect accuracy. Overcoming this challenge requires robust algorithms for dynamic lighting to ensure stable and precise localization and mapping.


The method proposed in \cite{cheng2021hierarchical} tackles the challenge of illumination changes using a deep descriptor network called a Dual Desc, which is designed to be robust against various appearance variations including illuminance changes. The network uses multimodal images (RGB, Infrared, and Depth) to generate robust attentive global descriptors and local features. These descriptors were used to retrieve coarse candidates of query images, and 2D local features, along with a 3D sparse point cloud, were used for geometric verification to select the optimal results from the retrieved candidates. The authors mentioned that their dataset included images captured at different times of the day, resulting in illumination changes between the query and database images. Despite these changes, the proposed method achieved satisfactory localization results. 


The authors of \cite{liu2020indoor} evaluated the influence of lighting conditions on the performance of their novel localization method. The authors captured training images during the day and test images at night, and simulated changes in lighting conditions by switching some of the lights off in locations without windows. The results showed that changes in the lighting conditions had a minor impact on the proposed method.
\cite{zhou2022multi} mentioned that the proposed localization scheme was verified in a typical office building environment with dramatically changing lighting conditions throughout the day; however, it does not provide detailed results or discussion on how changing lighting conditions affect the performance of the system.


The method proposed in \cite{salihappearance} addressed changes in illumination as a challenge using the COLD and IDOL datasets, which were recorded under different weather and illumination conditions (cloudy, night, and sunny) using different mobile platforms and camera setups. These datasets were used to evaluate the strength of the localization and recognition algorithms with respect to the variations caused by human activities and changes in illumination conditions. The study also mentioned the use of Histogram of Oriented Gradients (HOG) for feature extraction, which provides preferable invariant results for lighting or shadowing.


%
% Motion blur
%
\textbf{Motion blur}
Blurred images in visual SLAM can lead to inaccuracies in feature detection and matching, causing issues with pose estimation, map-building, loop closure, and visual odometry. These inaccuracies can also impact depth measurements and map quality. To address this issue, strategies such as using high-frame-rate sensors, incorporating IMUs, and employing motion deblurring techniques can be employed to improve the accuracy of localization and mapping in SLAM systems.
Motion blur can be caused by fast or sudden movements of the user during navigation, which can affect localization performance. \cite{liu2020indoor} studied this challenge and evaluated the robustness of the localization methods. They captured 2316 blurred images on the testing day. The results showed that the proposed method performed poorly in this experiment, indicating that fast motion or sudden changes in user movement can pose a challenge to the system. The reason for this poor performance was that the object detection scores did not exceed the threshold during the experiment.

%
% RQ4
%
\subsection{RQ4. How the proposed solution is expected to enhance mobility and navigation for visually impaired?}
This section discusses how the approaches proposed by the studies included in our SLR have the potential to improve navigation for BVI people.  These studies focused on diverse attributes, such as accurate pose estimation, semantic mapping, sensor fusion, and algorithmic innovations, to improve the quality of BVI navigation. Table \ref{rq4_mobility_improvement} presents the categorization of attributes that contribute to enhancing the mobility and navigation of visually impaired individuals.

SLAM technology is primarily used to provide precise localization, which is critical for assistive navigation systems. Precise localization provides accurate information regarding a user's position in the environment in which the user navigates. This accuracy enables the system to offer feedback on obstacles, pathways, and points of interest, thereby allowing BVI to navigate safely and confidently. Real-time assistance has also emerged as the key feature. Providing immediate feedback on the environment enables users to travel efficiently and safely, which leads to increased mobility and independence. 
Semantic mapping generates maps beyond geometric data. Such representations contain not only spatial information but also the semantic meanings of objects and features within the environment. This semantic understanding offers a deeper insight into the environment. This contextual awareness is particularly beneficial for enhancing navigation accuracy, as it enables navigation systems to make decisions based on semantic context, improving obstacle avoidance, path planning, and overall navigation efficiency. 

By employing robotic systems such as small robots, smart canes, and sensor-equipped suitcases, some studies have provided guidance, obstacle avoidance capabilities, and increased spatial awareness, thereby effectively providing independent navigation for visually impaired individuals.
Smartphone-based solutions harness the ubiquitous nature of smartphones that are equipped with cameras and sensors. These solutions offer navigation assistance by using widely available and familiar devices.
Both indoor and outdoor navigation capabilities offer a seamless transition between environments, ensuring that users receive consistent support, regardless of the scene in which they navigate.
Innovative localization and mapping algorithms enhance navigation efficiency and effectiveness through tailored modifications of existing SLAM frameworks or through the creation of novel solutions. Ultimately, these advancements have led to an improved overall experience for individuals with visual impairment.
Although these studies focused on different features and attributes, they all aimed to enhance mobility, independence, and overall quality of life for BVI people.


% Table 14. Attributes of SLAM-based navigation systems that contribute to enhancing BVI navigation, along with referenced papers emphasizing
\input{texs/tables/t14_RQ4_mobility_improvement}





==> texs/back-up/bck-t_core_technical_features.tex <==
\begin{table*}[t]
    % \footnotesize
    \scriptsize
    \centering
    \caption{Comparison of core technical features for localization and mapping techniques, with a specific focus on sensor types, computing resources, and whether machine learning-based methods are employed for localization and mapping tasks.}
    \label{tab:core_technical_features}
    \setlength{\tabcolsep}{3pt}
    \begin{tabularx}{\textwidth}{ p{20pt} X X X X }
    \hline
    \rowcolor{yellow}
    \textbf{Ref.} & \textbf{Sensor type} & \textbf{Computing Resource} & \textbf{Localization} \& \textbf{Mapping Technique} & \textbf{ML-Based Localization and Mapping} \\
    \hline

    % 
    % part 1
    % 
    
    \cite{ahmetovic2023sonification} & Camera & Smartphone & Native AI library for iOS devices & Not explicitly mentioned \\
    \cite{li2022sensing} & RGB-D camera & Remote server & ORB-SLAM2 & $\bullet$ \\
    \cite{song2023mixture} & A depth, an RGB, and four gray scale cameras, an IMU & Hololens2 device, GPU  & Iterative Closest Point (ICP) for camera pose estimation, Kinect Fusion algorithm for real-time 3D reconstruction & Not explicitly mentioned \\
    \cite{zhang2023research} & Wheel encoder and LiDAR & Notebook PC & Cartographer & $\bullet$ \\
    \cite{yang2022unav} & RGB camera & Cloud server and Nvidia Jetson AGX Xavier & Visual place recognition, weighted averaging, and perspective-n-point (PnP) for localization, OpenVSLAM and Colmap to generate a topometric map & NetVLAD for global descriptors and SuperPoint for local descriptors \\
    \cite{zhou2022multi} & LiDAR & Not mentioned & Cartographer to build SLAM maps on each floor & $\bullet$ \\
    \cite{hou2022knowledge} & RGB-D camera & Jetson AGX Xavier & ORB-SLAM2 for localization; down-sampling, octomap, and 2D occupancy grid mapping for an accurate dense mapping & $\bullet$ \\
    \cite{plikynas2022indoor} & IMU, stereo and IR (depth) cameras & Cloud server & ORB-SLAM3 & $\bullet$ \\
    \cite{xie2022multi} & RGB-D camera & Raspberry Pi & ORB-SLAM & $\bullet$ \\
    \cite{qiu2022egocentric} & Monocular RGB & Not mentioned & ORB-SLAM3 to obtain ground-truth camera trajectory & $\bullet$ \\
    \cite{chen2021wearable} & RGB-D camera & High performance portable processor, cloud server & Semantic visual SLAM based on ORB feature to generate sparse, dense, and semantic maps & ENet for pixel-level semantic segmentation \\
    \cite{slade2021multimodal} & LiDAR & Raspberry Pi & BreezySLAM & $\bullet$ \\
    \cite{lu2021assistive} & LiDAR & Intel NUC computer & GMapping for mapping and estimating the destination's location & $\bullet$ \\
    \cite{hakim2021indoor} & RGB-D camera & Raspberry Pi3 B+ & Hector SLAM for building the environmental map and locating the user on the map & $\bullet$ \\
    \cite{zhang2021rgb} & RGB-D Camera, IMU & UP Board computer & A VIO system developed based on VINS-Mono & $\bullet$ \\
    \cite{cheng2021hierarchical} & RGB-D-IR camera & A portable computer, Nvidia Jetson TX2 & Hierarchical visual localization pipeline with deep descriptors, geometric verification, and sequence matching. & NetVLAD and Dense Desc for advanced descriptor extraction. \\
    \cite{liu2020indoor} & RGB-D camera & Odroid XU3 board, remote server & Off-the-shelf algorithm \cite{endres20133} for 3D indoor mapping; a two-stream ConvNet for topological localization. & ConvNet replaces BoW for semantic info; Inception-v3 enhances object recognition, aiding localization. \\
    \cite{jin2020combining} & Two monocular cameras & Not mentioned & Followed a similar structure as ORB-SLAM2. & $\bullet$ \\
    \cite{bai2019wearable} & RGB-D camera, IMU & A smartphone with Qualcomm Snapdragon 820 CPU 2.0 GHz & Vins-mono for indoor localization; ORB-SLAM2 and Vins-mono for building a indoor map repository. & $\bullet$ \\
    \cite{zhang2019arcore} & Smartphone's camera & A HUAWEI P20 smartphone with Kirin 970 CPU & Roberto Lopez Mendez ARCore SLAM as the base for visual odometry and area learning & Not explicitly mentioned \\
    \cite{bai2018virtual} & Fisheye and depth camera & An embedded CPU board & ORB-SLAM2 for the building of the virtual-blind-road (offline by a sighted person) and the localization (online) & $\bullet$ \\
    \cite{zhang2017indoor} & SwissRanger SR4000 3D camera & A Lenovo ThinkPad T430 laptop (Intel core i5-3320M 2.6GHz CPU, NVS 5400m with 96 CUDA core) & 2-step graph SLAM & $\bullet$ \\
    \cite{zhang2020plane} & SwissRanger SR4000 camera, IMU & Up Board computer & PAVIO: Fusing visual, inertial, and plane features for robust SLAM localization and mapping. & $\bullet$ \\
    \cite{albogamy2021sravip} & Encoder, IMU, laser distance sensor & Raspberry Pi 3 Model B and B+ & Gmapping for building a 2D occupancy grid map on the environment & $\bullet$ \\
    \cite{crabb2023lightweight} & iPhone 11 Pro camera and IMU & iPhone 11 Pro & ARKit VIO for relative movements; ARKit mapping for semantic labels; Monte Carlo localization & YOLOv2 for object detection to facilitate effective localization \\
    \cite{son2022wearable} & RGB-D camera, compass sensor & Jetson Xavier AGX, NVidia & FastSLAM for mapping, ORB-SLAM2 for local pose estimation in the pre-built map & An extra thread aligns predicted semantics with key features. \\
    \cite{hakim2019indoor} & LiDAR, ultrasonic sensor, Raspberry pi camera & Raspberry Pi3 B+ & Hector SLAM for constructing a 2D-map of the environments and localization & $\bullet$ \\
    \cite{goswami2023efficient} & RGB-D, IMU & Nvidia Jetson AGX Xavier microprocessor & RTAB-Map for semantic point cloud generation and global localization & MobileNetV2 with PPM for constructing semantic point cloud \\
    \cite{hao2022detect} & Monocular camera & Nvidia Jetson Xavier NX Developer kit & Visual SLAM for user movement estimation and stationary object localization & $\bullet$ \\
    \cite{kuribayashi2023pathfinder} & LiDAR, IMU & Nvidia RTX 3080 graphic board & Cartographer for constructing a LiDAR map & $\bullet$ \\
    \cite{agrawal2022novel} & RGB-D, IMU & Dell G15 laptop with an RTX 3060 GPU & SLAM implementation by RealSense for creating an initial 2D occupancy grid and estimating user pose & $\bullet$ \\
    \cite{rui2021multi} & RBG-D camera & Uzel US-M5422 edge server, Raspberry Pi 4B & Improved ORB-SLAM for generating a dense navigation map and real-time positioning & $\bullet$ \\
    \cite{ou2022indoor} & RGB-D camera & Laptop & Dynamic-SLAM based on ORB-SLAM2 for estimating user's ego-pose and building a static feature point map & Non-Prior dynamic object detection preceding local mapping \\

    % 
    % part 2
    % 
    \cite{jin2021wearable} & RGB-D camera, IMU & Google Pixel 3 smartphone & RGBD-VIO for mapping and accurately estimating the device's pose & $\bullet$ \\
    \cite{xu2021multi} & RealSense D435i camera & Remote server based on Intel i7-8700 CPU, nvidia GTX1080 GPU & ORB-SLAM2 for environmental mapping and positioning of the user & $\bullet$ \\
    \cite{lu2021personalized} & Google glasses camera & GPU server & OpenVSLAM for mapping and locating user's indoor positions & $\bullet$ \\
    \cite{kayukawa2020guiding} & LiDAR, IMU & Laptop & Cartographer for estimating the current location and direction of a user & $\bullet$ \\
    \cite{chen2020navigation} & RGB-D camera, IMU & Not mentioned & ORB-SLAM2 for mapping and localizing the user & $\bullet$ \\
    \cite{chen2020can} & RGB-D camera & Nvidia Jetson AGX Xavier processor & OpenVSLAM for robust mapping and localization in real time. & $\bullet$ \\
    \cite{fusco2020indoor} & iPhone 8's IMU and rear-facing camera & iPhone 8 & Visual-Inertial Odometry with sign recognition and geometric constraints. & Not explicitly mentioned \\
    \cite{zhang2019human} & RGB-D camera, IMU & UP Board computer & Visual-Inertial Odometry for 3D mapping and pose estimation & $\bullet$ \\
    \cite{zhao2019multi} & RGB-D, LiDAR & Laptop & Semantic SLAM based on a 2D SLAM technique for determining the corridor area and mapping to a semantic map & YOLOv3 for landmark detection, Places365 for place recognition \\
    \cite{weiss2020navigation} & Vuze+ camera & Not mentioned  & ORB-SLAM2 for generating 3D positions and 2D connectivity graph from Vuze+ footage & $\bullet$ \\
    \cite{ramesh2018real} & Monocular camera & Intel i7 processor & Non-filter based visual SLAM using trained objects as landmarks for localization & ACF detector for object detection to identify trained objects of interest for localization. \\
    \cite{eden2018indoor} & ZED camera & Nvidia Jetson TX2 & ZED camera's SLAM for navigating toward an aisle in a grocery store. & Not mentioned \\
    \cite{mulky2018autonomous} & Stereo camera, laser & Nvidia Jetson TX2, Raspberry Pi, and Arduino. & RTAB-MAP for obtaining fine-grained mapping of the 3D spatial world. & $\bullet$ \\
    \cite{lalonde2018localizing} & Monocular camera & Not mentioned & Visual odometry for user localization during street crossings & $\bullet$ \\
    \cite{zhang2017plane} & 3D time-of-flight camera , IMU & UP Board computer & Plane-aided visual-inertial odometry (PAVIO) for pose estimation of an robotic navigation aid & $\bullet$ \\
    \cite{chen2017ccny} & Wide-angle lens camera, gyroscope, accelerometers, and infrared sensor on Google Tango. & Google Tango & Google Tango's built-in SLAM for mapping the environment and localizing the user. & $\bullet$ \\
    \cite{bai2017cloud} & Stereo camera & Cloud server & Visual SLAM for mapping the environment and localizing the user.  & $\bullet$ \\
    \cite{endo2017indoor} & Monocular camera & A single CPU & LSD-SLAM for estimating the user's position and constructing a 3D environmental map & $\bullet$ \\
    \cite{yang2022seeway} & Camera, IMU, LiDAR & Smartphone & visual-inertial SLAM based pose estimation and 2D scene-graph map construction using iOS ARKit. & Not explicitly mentioned \\
    \cite{shahani2023methods} & Kinect camera & Not mentioned & LSD-SLAM for assessing the user's location and building an environmental map & $\bullet$ \\
    \cite{yun2018design} & Laser Range Finder (LRF) sensor & PC & Hector SLAM for map building and odometry calculation & $\bullet$ \\
    \hline
    \end{tabularx}
\end{table*}


==> texs/back-up/bck-t_effectiveness_in_real_world_scenarios.tex <==
\begin{table*}[t]
% \footnotesize
 \scriptsize
\centering
\caption{\textbf{Effectiveness of localization and mapping techniques in real-world scenarios as \textcolor{red}{implied/mentioned} by the literature. The robustness and accuracy levels reported in this table are extracted from each paper's context; each rating reflects conditions specific to that paper and is not necessarily superior or inferior to the other approaches. Thus, these values are not comparable due to differing conditions across the papers. NM indicates that the information is not explicitly mentioned in the paper.}}
\label{tab:t_effectiveness_in_real_world_scenarios}
\setlength{\tabcolsep}{3pt}
\begin{tabularx}{\textwidth}{p{20pt} >{\centering\arraybackslash}p{30pt} X X >{\centering\arraybackslash}p{50pt} X }
\hline
\rowcolor{yellow}
\textbf{Ref.} & \textbf{Working area} & \textbf{Localization \& mapping accuracy level} & \textbf{Robustness level} & \textbf{Considers dynamic object}  & \textbf{Running time} \\
\hline

% 
% part 1
% 
\cite{ahmetovic2023sonification} & Both & \textcolor{MyGoldenrod}{Moderate}: Support in measuring errors. & \textcolor{MyGoldenrod}{Moderate}: System evaluates errors reliably. & $\bullet$ & Not mentioned \\
\cite{li2022sensing}& Indoor & \textcolor{MyDarkGreen}{High}: Ensuring safe indoor navigation & \textcolor{MyDarkGreen}{High}: Utilizes robust ORB-SLAM2 technique for reliable feature matching and adaptive navigation. & $\bullet$ & Affected by 0.15-1 sec transmission time to remote server \\
\cite{song2023mixture} & Indoor & Not provide specific details & \textcolor{MyDarkGreen}{High}: Instant localization, robust map building & $\bullet$ & Real-time \\
\cite{zhang2023research} & Indoor & \textcolor{MyDarkGreen}{High}: Confirmed through user-guided tests & Not provide specific details & $\checkmark$ & Not mentioned \\
\cite{yang2022unav} & Indoor & \textcolor{MyDarkGreen}{High}: With an average error of less than 1 meter & \textcolor{MyDarkGreen}{High}: Combined advantages of OpenVSLAM and Colmap & $\bullet$ & \textcolor{MyCrimson}{High}: Average response time of 2 to 3 seconds for localization \\
\cite{zhou2022multi} & Indoor & \textcolor{MyDarkGreen}{High}: With 0.62m for 3D and 1.24m for 2D & \textcolor{MyDarkGreen}{High}: Cartographer for mapping with optimization techniques & $\bullet$ & \textcolor{MyGoldenrod}{Moderate}: For localization is under 0.25 seconds \\
\cite{hou2022knowledge} & Indoor & \textcolor{MyDarkGreen}{High}: Accurate mapping, guiding users precisely to target goals & \textcolor{MyDarkGreen}{High}: Reliable performance with accurate mapping & $\bullet$ & \textcolor{MyGoldenrod}{Moderate}: Some delays in mapping, but overall meets real-time requirements \\
\cite{plikynas2022indoor} & Indoor & \textcolor{MyGoldenrod}{Moderate}: Needs improved SLAM stability and accuracy due to scaling issues & \textcolor{MyDarkGreen}{High}: due to SLAM loop closing, real-time correction & $\bullet$ & Not mentioned \\
\cite{xie2022multi} & Indoor & \textcolor{MyGoldenrod}{Moderate}: Effective mapping and localization but has deviations and mismatches impacting overall accuracy & \textcolor{MyDarkGreen}{High}: The integration of ORB-SLAM with YOLO ensures robust navigation and obstacle detection in various environments & $\bullet$ & \textcolor{MyGoldenrod}{Moderate}: Real-time map-building but slow path planning \\
\cite{qiu2022egocentric} & Both & \textcolor{MyDarkGreen}{High}: Precise ground truth trajectories, with minimal absolute error & \textcolor{MyDarkGreen}{High}: Reliable trajectory extraction with low absolute error
 & $\checkmark$ & Not mentioned \\
\cite{chen2021wearable} & Indoor & \textcolor{MyDarkGreen}{High}: With centimeter-level accuracy & \textcolor{MyDarkGreen}{High}: Real-time performance, centimeter-level accuracy, semantic mapping integration, and resource optimization & $\bullet$ & Real-time performance ensured through careful computing power allocation \\
\cite{slade2021multimodal} & Both & \textcolor{MyDarkGreen}{High}: RMSE between 0.08 and 0.44 m, indicating high precision in indoor environments & \textcolor{MyDarkGreen}{High}: SLAM-based system navigated complex environments with precision and consistent success across multiple trials & $\bullet$ & SLAM operated at 1.4 Hz, which is sufficient for real-time use \\
\cite{lu2021assistive} & Both & \textcolor{MyCrimson}{Low}: SLAM struggles with dynamic environments & \textcolor{MyCrimson}{Low}: SLAM demonstrates vulnerability in dynamic environments, with unstable navigation and orientation errors compared to UWB positioning & $\checkmark$ & \textcolor{MyCrimson}{High}: Averaging 317 seconds for navigation tasks in a dynamic environment \\
\cite{hakim2021indoor} & Indoor & Not explicitly mentioned & \textcolor{MyDarkGreen}{High}: Hector SLAM algorithm ensures robust mapping and localization accuracy. & $\checkmark$ & Real-time \\
\cite{zhang2021rgb} & Indoor & \textcolor{MyDarkGreen}{High}: With significant error reduction and effective 2D mapping alignment. & \textcolor{MyDarkGreen}{High}: Enhanced by floor plan integration, error reduction techniques, and superior performance in real-time pose estimation. & $\bullet$ & Real-time \\
\cite{cheng2021hierarchical} & Outdoor & \textcolor{MyDarkGreen}{High}: Superior accuracy demonstrated across multiple indicators and challenging conditions. & \textcolor{MyDarkGreen}{High}: Demonstrates superior robustness, especially in the presence of dynamic objects and changing illumination. & $\checkmark$ & \textcolor{MyGoldenrod}{Moderate}: Meets real-time requirements on powerful devices, but slower on less capable hardware. \\
\cite{liu2020indoor} & Indoor & \textcolor{MyDarkGreen}{High}: Achieved 96.3\% localization accuracy; outperforms other models despite pre-training limitations. & \textcolor{MyDarkGreen}{High}: Demonstrates robustness through accurate SLAM technique, semantic mapping, and deep learning integration for indoor localization. & $\bullet$ & \textcolor{MyCrimson}{High}: Longer computational time due to increased complexity or resource requirements. \\
\cite{jin2020combining} & Indoor & \textcolor{MyDarkGreen}{High}: Demonstrates superior accuracy compared to ORB-SLAM2 in dynamic environments. & \textcolor{MyDarkGreen}{High}: Demonstrates robustness through advanced SLAM techniques for obstacle removal and dynamic environment adaptability. & $\checkmark$ & Not mentioned \\
\cite{bai2019wearable} & Indoor: SLAM; outdoor: GPS & \textcolor{MyDarkGreen}{High}: Indoor localization with pre-built maps. & \textcolor{MyDarkGreen}{High}: VSLAM for indoor navigation enhances robustness in GPS-degraded environments. & $\checkmark$ & A real-time performance (approximate 20 fps) on a smartphone. \\
\cite{zhang2019arcore} & Indoor & \textcolor{MyDarkGreen}{High}: Rigorous comparison and real-time reliance on CAD maps ensure precise localization. & \textcolor{MyDarkGreen}{High}: Advanced localization and flexible path planning for accurate and safe navigation. & $\bullet$ & Not mentioned \\
\cite{bai2018virtual} & Indoor & \textcolor{MyDarkGreen}{High}: Key-frame matching and fisheye camera enhance feature detection and accuracy. & \textcolor{MyDarkGreen}{High}: ORB-SLAM2 for precise localization and obstacle avoidance in effective indoor navigation. & Dynamic obstacle in experiment path & \textcolor{MyDarkGreen}{Low}: Visual SLAM and dynamic subgoal selection optimize efficiency for real-time localization and mapping. \\
\cite{zhang2017indoor} & Indoor & \textcolor{MyDarkGreen}{High}: Superior to plane-based graph SLAM & \textcolor{MyDarkGreen}{High}: Efficiently addresses all 6-DOF and outperforms traditional SLAM methods & $\bullet$ & 59.4 ms average per frame \\
\cite{zhang2020plane} & Indoor & \textcolor{MyDarkGreen}{High}: Demonstrated by superior performance in pose estimation accuracy and robustness in various environments. & \textcolor{MyDarkGreen}{High}: Enhanced by integrating plane features and employing a plane consistency check for accurate pose estimation. & $\bullet$ & Not mentioned \\
\cite{albogamy2021sravip} & Indoor & Not mentioned & Not mentioned & $\checkmark$ & Real-time \\
\cite{crabb2023lightweight} & Indoor & \textcolor{MyDarkGreen}{High}: Utilizes visual landmarks, real-time data analysis, addresses limiting factors & \textcolor{MyDarkGreen}{High}: Robust to superficial changes, requiring updates only for major structural alterations. & $\bullet$ & \textcolor{MyGoldenrod}{Moderate}: Impacted by the number and type of visual landmarks. \\
\cite{son2022wearable} & Outdoor & \textcolor{MyDarkGreen}{High}: Global pose estimation within 80 cm radius of ground truth; verified in real-world scenarios. & \textcolor{MyCrimson}{Low}: Navigation relies on SLAM-relative poses, prone to instability with changing or occluded features. & $\bullet$ & Real-time \\
\cite{hakim2019indoor} & Indoor & \textcolor{MyDarkGreen}{High}: Accurate localization and mapping demonstrated through real-time indoor experiments in static scenarios. & \textcolor{MyDarkGreen}{High}: Hector SLAM ensures robustness in complex indoor environments for accurate navigation in static scenarios. & $\bullet$ & Real-time \\
\cite{goswami2023efficient} & Indoor & \textcolor{MyDarkGreen}{High}: <1m position error, <5\degree orientation error & \textcolor{MyDarkGreen}{High}: Integration of semantic SLAM, optimization of semantic Point Clouds during loop closures & $\bullet$ & Real-time (typically under 10 seconds, faster near distinctive features) \\
\cite{hao2022detect} & Both & \textcolor{MyDarkGreen}{High}: With an error of less than 0.5 meter & \textcolor{MyDarkGreen}{High}: Integration object detection and visual SLAM for accurate navigation support. & $\bullet$ & Real-time (with initialization under 2 seconds and trajectory estimation under 1 second.) \\

% 
% Part 2
% 
\cite{kuribayashi2023pathfinder} & Indoor & \textcolor{MyDarkGreen}{High}: Cartographer SLAM and 360 LiDAR for precise real-time mapping. & \textcolor{MyDarkGreen}{High}: Cartographer ensures dynamic, real-time LiDAR mapping with efficient updates in unfamiliar environments. & $\bullet$ & Real-time \\
\cite{agrawal2022novel} & Indoor & \textcolor{MyDarkGreen}{High}: SLAM algorithm and low-drift IMU enable precise user pose estimation and environment mapping. & \textcolor{MyDarkGreen}{High}: With real-time updates and effective threshold management. & $\bullet$ & \textcolor{MyDarkGreen}{Low}: Navigation completed within 45 seconds on average, well under the 2.5-minute cut-off. \\
\cite{rui2021multi} & Indoor & \textcolor{MyDarkGreen}{High}: Highly accurate in real-time testing & \textcolor{MyDarkGreen}{High}: Integrating ORB-SLAM and YOLO ensures stability and accuracy. & $\bullet$ & Not mentioned \\
\cite{ou2022indoor} & Indoor & \textcolor{MyDarkGreen}{High} accuracy feature-based visual SLAM estimation & \textcolor{MyGoldenrod}{Moderate}: Acknowledging limitations while utilizing effective techniques, indicating room for improvement. & $\checkmark$ & \textcolor{MyGoldenrod}{Moderate}: Accounting for variable GPU impact and dependency on tracked objects. \\
\cite{jin2021wearable} & Indoor & \textcolor{MyDarkGreen}{High} accuracy (RMSE 0.269), surpassing VINS-Fusion and VINS-RGBD. & \textcolor{MyDarkGreen}{High} robustness with RGBD-VIO, enhancing accuracy and efficiency for assistive navigation and object manipulation. & $\bullet$ & Not mentioned \\
\cite{xu2021multi} & Indoor & Achieving a 91\% success rate in navigation tasks & Demonstrating robustness, utilizing ORB-SLAM2 algorithm enables real-time path planning. & $\bullet$ & Real-time \\
\cite{lu2021personalized} & Indoor & Not specified & Not specified & $\bullet$ & Not mentioned \\
\cite{kayukawa2020guiding} & Indoor & \textcolor{MyDarkGreen}{High}: LiDAR and IMU data ensure precise localization and mapping. & \textcolor{MyDarkGreen}{High}: Integrating multiple sensors ensures robust localization for accurate navigation and collision avoidance. & $\checkmark$ & Not mentioned \\
\cite{chen2020navigation} & Likely indoor & \multicolumn{4}{c}{Lacking explicit discussion on accuracy, robustness, consideration of dynamic objects, and ML-based solutions.}\\
\cite{chen2020can} & Indoor & While numerical metrics are not mentioned, indicators suggest potential accuracy. & \textcolor{MyDarkGreen}{High}: OpenVSLAM framework ensures robust real-time mapping and localization capabilities. & $\bullet$ & Real-time \\
\cite{fusco2020indoor} & Indoor & \textcolor{MyDarkGreen}{High}: Consistently achieves sub-1 meter localization accuracy upon algorithm convergence. & \textcolor{MyDarkGreen}{High}: Utilizing stable landmarks and a particle filter ensures robust indoor localization. & $\bullet$ & Real-time operation with accurate localization post-algorithm convergence, demonstrating efficient performance on smartphones. \\
\cite{zhang2019human} & Indoor & \textcolor{MyDarkGreen}{High}: Achieving accurate pose estimation with a position error of 0.2 meters. & \textcolor{MyDarkGreen}{High}: Enhancing robustness with integrated VIO and Human Intent Detection for accurate pose estimation and mode selection. &$\bullet$ & \textcolor{MyDarkGreen}{Short}: Real-time pose estimation with updates every 22 milliseconds. \\
\cite{zhao2019multi} & Indoor (Corridor) & \textcolor{MyGoldenrod}{Moderate} Based on validation conducted in real-world scenarios & \textcolor{MyCrimson}{Low}: Performance degradation observed in specific scenarios due to narrow corridor and orientation estimation issues. & $\checkmark$ & Real-time \\
\cite{weiss2020navigation} & Outdoor & \multicolumn{4}{c}{SLAM used for localizing footage, creating spatial graphs, and generating realistic Deep Reinforcement Learning simulator data for pedestrian navigation training.} \\
\cite{ramesh2018real} & Indoor & \textcolor{MyDarkGreen}{High}: 94-98\% with relative errors of 1.6-2.6\% & \textcolor{MyDarkGreen}{High}: Efficient integration of visual SLAM, object detection, and depth measurements for precise, reliable indoor navigation. & $\bullet$ & Real-time \\
\cite{eden2018indoor} & Indoor & Not mentioned & Not mentioned & $\bullet$ & Not mentioned \\
\cite{mulky2018autonomous} & Both & \textcolor{MyDarkGreen}{High}: Accurate obstacle detection, extended range, minimal error in indoor mapping, integrated sensor data for dynamic environments. & \textcolor{MyDarkGreen}{High}: Dynamic adaptation, effective in complex and crowded environments with moving obstacles. & $\checkmark$ & Not mentioned \\
\cite{lalonde2018localizing} & Outdoor & Approximately 12cm error in localization accuracy & \textcolor{MyDarkGreen}{High}: Robust in weakly textured environments & $\bullet$ & Not mentioned \\
\cite{zhang2017plane} & Indoor & \textcolor{MyDarkGreen}{High}: Superior pose estimation accuracy (mean End Point Error Norm (EPEN): 2.63\%) compared to a state-of-the-art VIO (mean EPEN: 6.06\%). & \textcolor{MyDarkGreen}{High}: More stable performance (standard deviation EPEN: 1.3\%) than a state-of-the-art VIO (standard deviation: 8.22\%). & $\bullet$ & Not mentioned \\
\cite{chen2017ccny} & Indoor & Not evaluated & Not evaluated & $\bullet$ & Real-time \\
\cite{bai2017cloud} & Both & \textcolor{MyDarkGreen}{High}: Precise image feature extraction and motion trajectory reconstruction & \textcolor{MyDarkGreen}{High}: Dependable for tracking position and orientation. & NM & Real-time \\
\cite{endo2017indoor} & Indoor & \textcolor{MyDarkGreen}{High}: Precise self-positioning and mapping with high accuracy in large-scale environments. & \textcolor{MyDarkGreen}{High}: Superior robustness compared to conventional monocular SLAM algorithms, ensuring quick and reliable calculations. & $\checkmark$ & Real-time \\
\cite{yang2022seeway} & Indoor & \textcolor{MyDarkGreen}{High}: Assessed via quantitative metrics and real-world tests, achieving low navigation error and high success rate. & \textcolor{MyDarkGreen}{High}: Utilizing robust visual-inertial SLAM with iOS ARKit for accurate real-time navigation and obstacle avoidance. & NM & Real-time per-frame pose estimation \\
\cite{shahani2023methods} & Both & Not mentioned & Not mentioned & $\checkmark$ & Not mentioned \\
\cite{yun2018design} & Indoor & Not directly mentioned & \textcolor{MyGoldenrod}{Moderate}: Issues with mapping reflective or transparent surfaces like glass windows. & $\bullet$ & Not mentioned \\
\hline
\end{tabularx}
\end{table*}


==> texs/back-up/bck-t_limitations_potential_solutions.tex <==
\begin{table*}[t]
% \footnotesize
 \scriptsize
\centering
\caption{\textbf{A summary of perspectives and innovations in SLAM-based navigation solutions, with insights into limitations and advantages.}}
\label{tab:t_limitations_potential_solutions}
\setlength{\tabcolsep}{3pt}
\begin{threeparttable}
\begin{tabularx}{\textwidth}{p{20pt} >{\centering\arraybackslash}p{40pt} X X X X X }
\hline
\rowcolor{yellow}
\textbf{Ref.} & \textbf{Open-source} & \textbf{Research Issue} & \textbf{Contribution} & \textbf{Advantages}  & \textbf{Limitations} \\
\hline

% 
% Part 1
% 
\cite{ahmetovic2023sonification} & $\bullet$ & Addressing sonification techniques for navigation instruction & Innovative sonification for BVI navigation & Publicly available localization approach & Prone to drift, Utilizing markers for user positioning  \\
\cite{li2022sensing} & $\bullet$ & Enhancing indoor navigation for BVI with wearable technologies & Low-cost wearable, SLAM navigation, multitarget recognition & Non-intrusive wearable device, Map reuse, & Network impact, cognitive feedback needs \\
\cite{song2023mixture} & $\bullet$ & Improving perception and independent task completion for BVI & Mixed reality, real-time perception, remote assistance & Improves perception, functions in diverse indoors, advanced interactive platform, sensor integration & Network status influence \\
\cite{zhang2023research} & $\bullet$ & Addressing guide robots' lack of consideration for user status and obstacle properties & Introduced considerate robot design and spatial risk map for navigation & Robot adapts speed and movement, enhancing natural interaction without disturbing others; calculates pedestrian directions & Needs improved speech recognition, real-world testing with BVI, effective environmental interaction \\
\cite{yang2022unav} & $\bullet$ & Addressing limitations of sensor-based navigation for BVI & Infrastructure-independent vision-based navigation for BVI & Map-evolution feedback loop ensures dynamic updates, and offline computation allows for continued use during signal loss. & Requires a dense reference image database; difficult to adapt to diverse environments. \\
\cite{zhou2022multi} & $\bullet$ & Improving high-precision indoor localization in complex multi-floor environments & Hybrid localization framework combining visual and wireless signals for high-precision indoor localization & Multi-modal sensor integration, fusion-based localization, and GAN-based approach for efficient, high-precision multi-floor localization & Implementation complexity, low positioning accuracy, and dependence on fingerprint database and offline maps \\
\cite{hou2022knowledge} & $\bullet$ & Applying object-goal navigation to aid BVI in indoor settings & Migration of object-goal navigation to assistive devices and a knowledge-driven approach & Active assistance with context-aware, knowledge-driven navigation for improved indoor object-goal guidance & Dependency on unlabelled images, scene understanding complexity, and generalization to unfamiliar environments. \\
\cite{plikynas2022indoor} & $\bullet$ & Operationalizing Web 2.0 social networking for indoor navigation assistance & Innovative integration of Crowdsourcing and social networking for indoor navigation & Constant access to a 24/7 indoor route database, offline functionality, and flexible, user-friendly wearable devices & Relies heavily on social networking, high processing power, and stable Internet connectivity \\
\cite{xie2022multi} & $\bullet$ & Enhancing guidance systems for BVI with multi-sensory integration for improved indoor navigation & Integration of ORB-SLAM with YOLO, dense map generation, and practical prototype implementation & Obstacle avoidance with multi-sensory feedback, dense navigation maps, and real-time target detection, implemetation of a practical smart cane & Dense map may not always align with reality, pathfinding has high computational costs, and target detection is trained based on a generic dataset.
 \\
\cite{qiu2022egocentric} & \href{https://github.com/Jianing-Qiu/TISS}{Trajectory dataset} \tnote{1} &  Forecasting egocentric camera wearers' trajectories in crowded spaces & A new egocentric dataset, a Transformer-based model with cascaded cross-attention, and demonstration of socially compliant robot navigation & An egocentric view with multi-modal fusion for trajectory forecasting; Socially compliant robot navigation and assists visually impaired individuals. & Not mentioned \\
\cite{chen2021wearable} & $\bullet$ &  limited navigation options, wearable devices, semantic visual SLAM, cost-effective solutions & Semantic SLAM integration, real-time solution, efficient resource allocation & Real-time semantic understanding, efficient resource allocation, enhanced navigation accuracy, voice broadcast for destination assistance & Remote server challenges including internet access dependency, security, and privacy concerns \\
\cite{slade2021multimodal} & $\checkmark$ & Decreasing cognitive burden, increasing walking speed with a multimodal augmented cane & Improving mobility with sensors, intuitive steering, and advanced navigation features, increasing walking speed & Enhanced mobility, faster walking, precise steering, reduced cognitive load, fewer collisions, increased confidence, reliable obstacle avoidance, failure backup,  selecting preferred walking speed by user & Heavy, requiring mechanical assembly \\
\cite{lu2021assistive} & $\bullet$ & Enhancing navigation with improved robotic assistance in dynamic environments. & A novel haptic-guided robot with enhanced navigation, dynamic obstacle avoidance via UWB, and voice-enabled beacon feedback & Enhanced environmental information, intuitive navigation, precise UWB positioning, semantic feedback, and DRL-based obstacle avoidance. & Dynamic obstacles impact SLAM accuracy; implicit learning in the simulator may cause real-world uncertainties. \\
\cite{hakim2021indoor} & $\bullet$ & Efficient indoor navigation aid. & Multi sensor utilization, efficient algorithm utilization, and real-time voice guidance. & Cost-effective, real-time navigation, accurate mapping, obstacle detection, efficient path planning. & Limited to static, simple environments. \\
\cite{zhang2021rgb} & $\bullet$ & Enhancing navigation accuracy and robustness in large indoor spaces for assistive technologies. & Introduced DVIO for enhanced 6-DOF pose estimation and VPS for accurate assistive navigation. & Enhanced pose accuracy, real-time updates, effective wayfinding, obstacle avoidance, and significant pose error reduction. & Pose drift remains an issue in complex environments. \\
\cite{cheng2021hierarchical} & $\bullet$ & Improving visual localization in challenging outdoor settings. & Unified Dual Desc network enhancing descriptor extraction and multimodal integration for assistive localization. & Enhances robustness using multimodal imaging, advanced descriptors, and sequential integration for outdoor navigation. & Lacks real-time execution capability in assistive device. \\
\cite{liu2020indoor} & $\bullet$ & Enhancing independence for visually impaired through semantic environmental understanding and navigation. & Integrates ConvNets for semantic mapping; enhances topological localization. & Enhanced accuracy, semantic guidance, robustness to changes. & Computational inefficiency, suboptimal performance in motion blur effects. \\
\cite{jin2020combining} & $\bullet$ & Addressing the lack of comprehensive solutions for indoor navigation and obstacle avoidance. & Integration of dynamic person-detection method (EER–ASSL) and VSLAM for real-time navigation assistance in cluttered environments. & Enhanced smooth movement, reliable obstacle avoidance, effective navigation in dynamic environments. & Limited instruction capabilities, the decrease in person detection performance under varying lighting conditions and speed. \\
\cite{bai2019wearable} & $\bullet$ & Addressing lack of integrated navigation and object recognition systems. & Integration of lightweight CNN-based object recognition and visual SLAM for improved environment perception and navigation. & Load cognitive decrease, safe and quick navigation, enhanced perception, and real-time performance on smartphones. & Unable to detect small-size obstacles and obstacle detection limitations. \\
\cite{zhang2019arcore} & $\bullet$ & Addressing lack of user-centric indoor navigation aids for visually impaired. & ARCore integration, adaptive path planning, and dual-channel user interaction for indoor navigation. & Enhanced mapping, obstacle-avoiding path planning, and intuitive dual-channel interaction for improved indoor navigation. & Reliance on existing indoor scenario CAD maps. \\
\cite{bai2018virtual} & $\bullet$ & Addressing gaps in localization, way-finding, and route following for visually impaired navigation. & Dynamic subgoal route following, visual SLAM integration, and wearable optical see-through glasses for enhanced indoor navigation. & Enhances precision with visual SLAM, cost-effective sensors, efficient obstacle avoidance, safe indoor navigation with dynamic subgoal selection. & Not mentioned \\


% 
% part 2
% 
\cite{zhang2017indoor} & $\bullet$ & Addressing accumulative pose error, GPS-denied navigation, and real-time pose estimation. & New 6-DOF pose estimation method using floor and wall information, and a real-time wayfinding system. & Reduces accumulative pose error and provides real-time wayfinding  & System less effective in simple tasks, weight causes discomfort, and fails at high walking speeds over 0.6 m/s. \\
\cite{zhang2020plane} & $\bullet$ & Addressing accurate 6-DOF pose estimation challenges through innovative visual-inertial odometry for robotic navigation aids. & A plane-aided VIO method and a plane-consistency check for enhanced pose estimation accuracy. & Improved accuracy, a plane-consistency check, practical implementation for assistive navigation, and outperformance of state-of-the-art methods. & Not mentioned \\
\cite{albogamy2021sravip} & $\bullet$ & Enhancing navigation in an indoor public environment for pre-scheduled tasks with user-independent robotic solutions. & Innovative user-independent robotic assistance for indoor navigation. & Enhancing inclusivity and efficiency: user-independent robotic assistance. & It is not mentioned how the proposed approach handles crowds in the public places under study. \\
\cite{crabb2023lightweight} & \href{https://www.openicpsr.org/openicpsr/project/183714/version/V1/view}{ICOSR repository} \tnote{2} & Developing a lightweight indoor localization system using a 2D floor plan of the environment rather than a 3D model. & Innovative localization algorithm integrating visual landmarks, VIO, and 2D floor plans. & Smartphone-based, lightweight, and robust localization approach. & Noisy distance estimates due to imprecise bounding boxes. \\
\cite{son2022wearable} & Raw data supporting the conclusion & Addressing the need to ensure safe street crossing & Introducing a comprehensive wearable system for safe urban navigation, integrating real-time computer vision and prior maps. & Utilizes pre-built LiDAR maps, such as those publicly available and created for autonomous vehicles, supports user's preferred walking speed. & Dependent on specific crosswalk textures, lacks dynamic obstacle handling, may face instability with changing features, and outdoor noise interference. \\
\cite{hakim2019indoor} & $\bullet$ & Integration of navigation and object recognition. & Integration of navigation, object recognition, and low-cost sensors. & Integrated navigation and object recognition, low-cost sensors, efficient path planning, accurate real-time object identification in static scenarios. & Restricted to static simple environments. \\
\cite{goswami2023efficient} & $\bullet$ & Enhancing real-time global indoor localization using Semantic SLAM and a priori maps for GPS-deprived environments. & Implementing vector-based semantic extraction from floor plans, efficient particle filter localization, and leveraging loop closures for active semantic point cloud. & Real-time, accurate localization; integration of semantic information; using deep learning for enhanced robustness and efficiency. & Visual aliasing, limited semantic classes. \\
\cite{hao2022detect} & $\bullet$ & Addressing navigation challenges for BVI by developing a wearable solution for real-time guidance to target objects in unfamiliar settings. & Introducing a wearable navigation system with real-time object localization, visual SLAM, and trajectory estimation for efficient user guidance. & High accuracy, vision-based, real-time assistance, continuous object tracking, and portable system design. & Not explicitly mentioned. \\
\cite{kuribayashi2023pathfinder} & $\bullet$ & Addressing the challenge of navigation in unfamiliar indoor spaces by designing a map-less system, PathFinder & Developing a map-less navigation robot system incorporating sign recognition and intersection detection, using scenario-based participatory design with five blind participants. & Enhanced navigation confidence, provided key sign information, offered audio feedback, ensured safe, independent mobility by PathFinder & Limited study environments, assumed environments without steps or floor transitions, no empirical comparison with participants' regular aids, inability to recruit younger participants and insufficient number of guide dog users, possible positive bias from participants who have previously participated in studies, physical demand, Bluetooth connectivity issues, privacy concerns, inability to navigate in congested spaces, surrounding people may not recognize that users are disabled as they don’t use traditional aids. \\
\cite{agrawal2022novel} & $\bullet$ & Enhancing independent navigation and social seat selection with a perceptive robotic cane system. & Introducing a robotic cane with computer vision for navigation and social seat selection, featuring vibrotactile feedback and successful pilot validation. & Independent navigation, social norm-aware seat selection, intuitive vibrotactile feedback, and effective pilot-validated guidance. & Potential suboptimal chair detection, discrepancy between user preferences and performance. \\
\cite{rui2021multi} & $\bullet$ & Overcoming limitations of existing blind navigation methods by integrating multi-sensory feedback for comprehensive and intuitive mobility. &  Integration of YOLO and ORB-SLAM, enhanced by novel algorithms, provides reliable multi-sensory guidance & Enhanced accuracy, multi-sensory feedback, real-time object detection, dense navigation maps, and comprehensive guidance improve mobility and safety. & Not explicitly mentioned \\
\cite{ou2022indoor} & $\bullet$ & Addressing gap: aiding visually impaired in dynamic indoor navigation, obstacle detection, and social distancing. & Wearable RGB-D assistant system aiding indoor localization, mapping, and dynamic obstacle detection. & Dynamic object detection, enhanced obstacle avoidance, panoptic segmentation for scene understanding, robust tracking without additional models, and RGB-D sensor integration. & Imperfect panoptic segmentation, leading to errors in object recognition; computational complexity, influenced by the number of dynamic objects present in the scene.\\
\cite{jin2021wearable} & $\bullet$ & Addressing the gap: wearable device aiding visually impaired with indoor object manipulation tasks. & Hand-worn assistive device, RGBD-VIO method, effective human-device interface. & Enhanced pose estimation, depth information utilization, improved human-device interaction, effective object manipulation. & Not mentioned \\

% 
% part 3
% 
\cite{xu2021multi} & $\bullet$ & Addressing the challenge of indoor navigation, integrating SLAM and deep learning enhances environmental perception. & Introducing multi-functional smart E-Glasses for enhanced indoor navigation and lightweight object detection. & Real-time navigation, high object detection precision, and robust SLAM integration. & Future enhancements aim to improve device comfort, portability, and size, addressing user concerns and enhancing overall usability. \\
\cite{lu2021personalized} & $\bullet$ & Addressing the gap in understanding between visually impaired individuals' perceptions and their actual surroundings for navigation technology. & Introducing personalized navigation system with object detection and description, and re-training models. & Personalized navigation, object detection, reduced time for finding destinations, and improved interaction. & Model re-training challenges, environmental complexity, and high computational cost. \\
\cite{kayukawa2020guiding} & $\bullet$ & Addressing the need for a guiding system to facilitate seamless walking in public spaces. & Introducing a comprehensive system aiding blind pedestrians by understanding nearby pedestrians' behavior. & Convenient suitcase design, accurate motion tracking, effective tactile interface for enhanced navigation. & Weight discomfort, space constraints, speed adjustment difficulties, and technological improvements for enhanced usability. \\
\cite{chen2020navigation} & $\bullet$ & Addressing the need for advanced navigation aid for the visually impaired using VSLAM technology. & Introducing a navigation aid system merging VSLAM with pre-established maps. & Not explicitly mentioned & Not explicitly mentioned \\
\cite{chen2020can} & $\bullet$ & Addressing the need for unified indoor navigation, integrating scene perception and visual localization. & Introducing a unified semantic visual localization system, enhancing obstacle avoidance and spatial awareness. & Real-time awareness, comprehensive understanding, and obstacle avoidance. & Restricted camera field of view and inconsistencies in semantic segmentation results impacting user confidence. \\
\cite{fusco2020indoor} & Upon publication & Addressing indoor navigation challenges through smartphone-based computer vision without new infrastructure. & Real-time app development, robust localization algorithm, and user-friendly navigation. & Cost-effective deployment, enhances usability, improves localization accuracy, promises full-featured wayfinding, and camera-agnostic navigation for ease of use. & Challenges in wide, open indoor spaces due to limitations in current approach, suggesting potential for augmented reality integration. \\
\cite{zhang2019human} & $\bullet$ & Addressing the indoor wayfinding problem & Introducing specialized robotic navigation aid, VIO method, guiding modes, and Human Intent Detection for enhanced navigation assistance. & Enhanced VIO method, two guiding modes, and automated mode selection. & Validation in larger spaces, user feedback incorporation, and operational restrictions. \\
\cite{zhao2019multi} & $\bullet$ & Addressing independent indoor corridor navigation through multi-sensor fusion and semantic mapping. & Semantic mapping, multi-sensor fusion, real-time performance enhancement & Enhanced corridor navigation, semantic mapping, landmark detection, real-time performance, multi-sensor fusion for improved navigation experience. & Object recognition limitations, arrow direction detection issue, training requirement for unknown objects. \\
\cite{weiss2020navigation} & \href{https://github.com/mweiss17/SEVN-data}{SEVN-data} \tnote{3} & Enhancing Reinforcement Learning environments to develop a navigation assistant tailored for the BVI community. & Developing a benchmark dataset and Reinforcement Learning training environment to advance navigation agent capabilities using real-world imagery and neural architecture. & SEVN offers realistic training with a rich, annotated dataset and a multi-modal fusion model for effective BVI navigation. & SEVN provides an open, extensible Reinforcement Learning environment for BVI navigation, with potential for improved model performance through enhanced data and technology integration. \\
\cite{ramesh2018real} & $\bullet$ & Addressing real-time localization and navigation in indoor settings with a monocular camera, focusing on computational efficiency, user-friendly interfaces, and integrated algorithms. & Introducing a non-filter based visual SLAM with integrated object detection and distance-depth estimation algorithms, using a single monocular camera for BVI indoor navigation. & Utilizing a single camera and simpler SLAM algorithm for cost-effective, efficient real-time performance. & Not mentioned \\
\cite{eden2018indoor} & $\bullet$ & Enhancing indoor localization for visually impaired shoppers using text extraction, addressing gaps in traditional visual assistance systems. & Expanding SLAM algorithm for larger spaces using GIST/SURF features and navigating through text-rich environments. & Simplistic setup, no markers needed, and efficient real-time localization. & Operates only within length dimension of the aisle, limited by text density. \\
\cite{mulky2018autonomous} & Android APIs & Enabling safe autonomous navigation for elderly and visually impaired in crowded environments. & Design of an intelligent autonomous scooter with advanced sensor fusion, SLAM techniques, and hybrid mapping solutions. & Improved safety and autonomy, hybrid mapping for diverse environments, precise steering control. & Not mentioned \\
\cite{lalonde2018localizing} & $\bullet$ & Localizing pedestrians in crosswalks using visual odometry, addressing challenges in uniform textures and repetitive landmarks. & Introducing a prototype for localizing pedestrians in crosswalks using visual odometry. & Accurate on weakly textured surfaces, addressing scaling issues in monocular camera setups. & Initialization issues, tracking loss due to strong orientation variations, and challenges with oscillatory walking patterns. \\
\cite{zhang2017plane} & $\bullet$ & Improving indoor pose estimation accuracy for navigation aids using plane features in feature-sparse environments. & Introducing PAVIO method, utilizing plane features and factor graph optimization to improve pose estimation for indoor navigation. & Improved pose estimation accuracy and robustness, enhanced stability, accurate 3D mapping. & Not mentioned \\
\cite{chen2017ccny} & $\bullet$ & Addressing indoor navigation challenges to enhance mobility and independence. & Implementation of SmartCane with Google Tango for real-time indoor navigation and demonstration of its effectiveness in aiding visually impaired users. & Enhanced indoor navigation with real-time path planning, multimodal feedback, and an intuitive control panel interface. & Requiring further user evaluation to assess effectiveness \\

%
% part 4
%
\cite{bai2017cloud} & $\bullet$ & Developing a cloud and vision-based system for safe navigation and detailed perception. & Integrating cloud computing with vision-based navigation, enhancing perception, and improving object recognition for blind individuals. & Detailed perception, real-person safety support, abundant surrounding information, and improved object recognition. & Requiring extensive vision-based mapping, struggles with similar scenarios, and needs improved scene parsing, currency validation, and object recognition. \\
\cite{endo2017indoor} & $\bullet$ & Addressing the need for specialized navigation systems for visually impaired individuals using SLAM technology for real-time guidance. & Introducing a wearable camera with LSD-SLAM for real-time positioning, obstacle detection, and route guidance. & Efficient calculation power, robust performance, accurate mapping, dynamic adaptation, real-time assistance. & Requires high-contrast environments for accurate mapping; low contrast may need external positioning solutions. \\
\cite{yang2022seeway} & $\bullet$ & Addressing the need for an innovative navigation system using vision-language model-based approach. & First BVI navigation system using spoken instructions, visual-language integration, and heuristic-based path planning for improved success. & Running on portable devices, provides BVI navigation without heavy labeling or 3D model reconstruction in complex indoor environments. & Navigation reliability drops for long distances. \\
\cite{shahani2023methods} & $\bullet$ & Addressing real-time navigation latency, safe route selection, and accurate obstacle detection. & Integration of Web of Things, predictive analytics, YOLOv4 Tiny, and SLAM for enhanced obstacle recognition and navigation. & Enhanced obstacle recognition, navigation, and safe route selection. & Requiring high-contrast environments; needing external updates when contrast is insufficient for accurate mapping. \\
\cite{yun2018design} & $\bullet$ & Addressing the need for efficient navigation solutions for visually impaired individuals and patients with lower body injuries indoors. & Developed a person carrier robot integrating Hector SLAM and Robust Salient Detection for safe navigation and obstacle avoidance. & Enhanced safety, improved mobility, and effective object detection for indoor navigation. & Sensitive to strong light, issues with reflective surfaces, and occasional collisions due to slow processing speed. \\
\hline
\end{tabularx} 
     \begin{tablenotes}
    \item[1] \url{https://github.com/Jianing-Qiu/TISS} (Accessed on 3 May 2024)
    \item[2] \url{https://www.openicpsr.org/openicpsr/project/183714/version/V1/view} (Accessed on 3 May 2024)
    \item[3] \url{https://github.com/mweiss17/SEVN-data} (Accessed on 12 May 2024)
    \end{tablenotes}
\end{threeparttable}
\end{table*}


==> texs/back-up/bck-t_practical_challenges.tex <==
\begin{table*}[t]
% \footnotesize
 \scriptsize
\centering
\caption{\textbf{Practical challenges and Operational efficiency. The information in this table has either been directly extracted from the article or can be easily inferred from the article's text. - indicates that the information is not specified in the respective papers.}}
\label{tab:practical_challenges}
\setlength{\tabcolsep}{3pt}
\begin{tabularx}{\textwidth}{p{20pt} p{60pt} >{\centering\arraybackslash}p{50pt} >{\centering\arraybackslash}p{50pt} X X X X X X }
\hline
\rowcolor{yellow}
 \multirow{2}{*}{\textbf{Ref.}} & \multirow{2}{*}{\textbf{Assistive tool}} & \multicolumn{2}{c}{\textbf{User-friendliness}} & \textbf{Cost-efficient} & \textbf{Weight} & \textbf{Comfort for extended use} & \textbf{Adjustable fit} & \textbf{Fatigue mitigation} & \textbf{Portability} \\
 \cline{3-4}
 & & \textbf{Clear instructions} & \textbf{Easy to learn} &  &  &  &  &  &  \\
\hline

% 
% part 1
% 

\cite{ahmetovic2023sonification} & Smartphone & $\checkmark$ & $\checkmark$ & - & - & - & - & - & - \\
\cite{li2022sensing} & Electronic glasses and leg-mounted haptic modules & $\checkmark$ & - & $\checkmark$ & Light & $\checkmark$ & $\checkmark$ & $\checkmark$ & \textcolor{MyDarkGreen}{High} \\
\cite{song2023mixture} & Microsoft Hololens2 & $\checkmark$ & - & - & Light & - & $\checkmark$ & - & \textcolor{MyDarkGreen}{High} \\
\cite{zhang2023research} & Wheeled guide mobile robot & $\checkmark$ & - & - & Light & $\checkmark$ Easy-to-hold handle & - & - & \textcolor{MyGoldenrod}{Moderate} \\
\cite{yang2022unav} & Android application & $\checkmark$ & - & $\checkmark$ & Light & $\checkmark$ & $\checkmark$ & $\checkmark$ & \textcolor{MyDarkGreen}{High} \\
\cite{zhou2022multi} & \multicolumn{9}{c}{Not a user-based evaluation: only a technical test.} \\
\cite{hou2022knowledge} & Helmet; white cane & $\checkmark$ & - & - & Light & $\checkmark$ & - & - & \textcolor{MyGoldenrod}{Moderate} \\
\cite{plikynas2022indoor} & Smartphone & $\checkmark$ & Need time to learn interpreting tactile signals  & - & - & - & - & - & - \\
\cite{xie2022multi} & Smart cane & $\checkmark$ & - & - & Light & - & - & - & \textcolor{MyDarkGreen}{High} \\
\cite{qiu2022egocentric} & \multicolumn{9}{c}{No prototype implemented; the proposed approach for trajectory forecasting was tested with a robot.} \\
\cite{chen2021wearable} & A forehead-mounted camera, an earphone, a computing resource bag & \multicolumn{2}{c}{Not a user-based evaluation: only a technical test performed.} & $\checkmark$ & \textcolor{MyCrimson}{Heavy} & Heavyweight & - & Heavyweight & \textcolor{MyGoldenrod}{Moderate} \\
\cite{slade2021multimodal} & Augmented cane & $\checkmark$ & $\checkmark$ & $\checkmark$ & \textcolor{MyCrimson}{Heavy} (1kg) & Heavyweight & $\checkmark$ & Heavyweight & \textcolor{MyGoldenrod}{Moderate} \\
\cite{lu2021assistive} & Guiding robot & $\checkmark$ & $\checkmark$ & USD 17000 & \textcolor{MyCrimson}{Heavy} (25kg) & Comfortable handle feedback; some users noted slewing and speed change discomfort. & - & - & The robot is relatively large at 41x43x25 $\mathrm{cm}^3$. \\
\cite{hakim2021indoor} & Head-mounted camera & \multicolumn{2}{c}{Not a user-based evaluation: only a technical test performed.} & $\checkmark$ & Light & - & - & - & - \\
\cite{zhang2021rgb} & Smart cane & \multicolumn{8}{c}{Not a user-based evaluation: only a technical test performed.} \\
\cite{cheng2021hierarchical} & Auxiliary glasses & \multicolumn{8}{c}{Not a user-based evaluation: only a technical test performed.} \\
\cite{liu2020indoor} & \multicolumn{9}{c}{No prototype implemented: Only a technical test performed.} \\
\cite{jin2020combining} & Smart eyeglasses & Limited instructions & - & $\checkmark$ & - & - & - & - & \textcolor{MyDarkGreen}{High} \\
\cite{bai2019wearable} & Eyeglasses-mounted sensors + smartphone & $\checkmark$ & Participants trained in 10 minutes & $\checkmark$ & Light & Prolonged beeping may cause discomfort. & - & Glasses weight strains the nose. & \textcolor{MyDarkGreen}{High} \\
\cite{zhang2019arcore} & ARCore-supported smartphone + haptic gloves & $\checkmark$ & A 5-minute tutorial & $\checkmark$ & - & - & - & - & \textcolor{MyDarkGreen}{High} \\
\cite{bai2018virtual} & Optical see-through glasses & - & - & $\checkmark$ & - & - & - & - & \textcolor{MyDarkGreen}{High} \\
\cite{zhang2017indoor} & Smart cane & - & - & - & \textcolor{MyCrimson}{Heavy} & Low comfort & - & Heavyweight & \textcolor{MyCrimson}{Low}: Bulky tablet hangs on neck, heavy cane \\
\cite{zhang2020plane} & Computer-vision-enhanced white cane & \multicolumn{8}{c}{Not a user-based evaluation: only a technical test performed.} \\
\cite{albogamy2021sravip} & Smart robot & \multicolumn{8}{c}{No information available.} \\
\cite{crabb2023lightweight} & Smartphone & \multicolumn{2}{c}{Not mentioned} & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ & \textcolor{MyDarkGreen}{High} \\
\cite{son2022wearable} & Head-worn camera & Easily understood commands & 10-minute training & Commercially available hardware & \textcolor{MyCrimson}{Heavy} (5.5lbs $\approx$ 2.49kg) & - & - & - & \textcolor{MyDarkGreen}{High} \\
\cite{hakim2019indoor} & Sensors attached to a white cane & \multicolumn{2}{c}{Not a user-based evaluation.} & $\checkmark$ & \multicolumn{5}{c}{Not a user-based evaluation: only a technical test performed.} \\
\cite{goswami2023efficient} & \multicolumn{9}{c}{No prototype implemented; the proposed approach for real-time global localization was tested with an agent.} \\
\cite{hao2022detect} & Chest-mounted camera & \multicolumn{2}{c}{Not a user-based evaluation} & $\checkmark$ & Light & \multicolumn{3}{c}{Not explicitly mentioned.} & \textcolor{MyDarkGreen}{High} \\
\cite{kuribayashi2023pathfinder} & Suitcase-shaped robot & Improved with intuitive terminology & Positive usability scores & - & \textcolor{MyCrimson}{Heavy} (40lbs $\approx$ 18.14 kg) & Physical demand & - & Heavyweight & \textcolor{MyCrimson}{Low}: Bulky and heavy \\
\cite{agrawal2022novel} & Robotic cane & - & - & - & - & - & - & - & Self-contained and portable \\
\cite{rui2021multi} & Smart cane & \multicolumn{7}{c}{The focus of the paper is primarily on the technical aspects of the multi-sensory blind guidance system. } \\
\cite{ou2022indoor} & Smart glasses & - & - & - & Light & - & - & - & - \\
\cite{jin2021wearable} & Hand-worn device & \multicolumn{2}{c}{Not a user-based evaluation: only a technical test performed.} & - & 52.5 grams & - & - & - & - \\

% 
% part 2
% 
\cite{xu2021multi} & Smart E-glasses & - & - & - & - & Areas for improvement & - & - & - \\
\cite{lu2021personalized} & Google glasses & \multicolumn{8}{c}{Information not provided; Only a technical test conducted with a laptop PC as a navigator.} \\
\cite{kayukawa2020guiding} & A rolling suitcase-shaped device & $\checkmark$ & Short training session (10-20 minutes) & - & \textcolor{MyCrimson}{Heavy} & Weight discomfort & - & Heavy and bulky & Space limitations \\
\cite{chen2020navigation} & \multicolumn{9}{c}{System testing was not feasible as the system was in the experimental stage.} \\
\cite{chen2020can} & Smart glasses & \multicolumn{8}{c}{Not a user-based evaluation: only a technical test performed.} \\
\cite{fusco2020indoor} & Smartphone & $\checkmark$ & $\checkmark$ & $\checkmark$ & Light & $\checkmark$ & $\checkmark$ & $\checkmark$ & High \\
\cite{zhang2019human} & White-cane mounted camera & \multicolumn{8}{c}{Information not provided; Only a technical test performed.} \\
\cite{zhao2019multi} & TurtleBot2 robot (to be replaced by portable device) + wearable sensors& - & - & - & \textcolor{MyCrimson}{Heavy} & Heavy and bulky & - & - & Bulky \\
\cite{weiss2020navigation} & \multicolumn{9}{c}{Paper develops a Reinforcement Learning environment to create a navigation assistant tailored for the BVI community, without user-based evaluation.} \\
\cite{ramesh2018real} & Smartphone & - & - & $\checkmark$ & Light & $\checkmark$ & $\checkmark$ & $\checkmark$ & High \\
\cite{eden2018indoor} & \multicolumn{9}{c}{No prototype implemented; the proposed approach was tested within a research building.} \\
\cite{mulky2018autonomous} & Intelligent autonomous scooter & - & - & High cost & \textcolor{MyCrimson}{Heavy} & - & - & - & Bulky \\
\cite{lalonde2018localizing} & Wearable camera & - & - & - & Light & - & - & - & High \\
\cite{zhang2017plane} & Computer-vision-enhanced white cane & \multicolumn{8}{c}{Not a user-based evaluation: only a technical test performed.} \\
\cite{chen2017ccny} & Smart cane + Google Tango & - & - & - & 225 grams & - & - & - & \textcolor{MyDarkGreen}{High}: light and compact, usable in multi-floor \\
\cite{bai2017cloud} & Helmet-mounted camera + android-based smartphone & \multicolumn{8}{c}{Not a user-based evaluation: only a technical test performed.} \\
\cite{endo2017indoor} & Wearable camera & \multicolumn{8}{c}{Not a user-based evaluation: only a technical test performed.} \\
\cite{yang2022seeway} & iPhone 12 Pro Max & Effective language instructions & Intuitive navigation process & - & Light & - & - & - & High \\
\cite{shahani2023methods} & Wearable camera & \multicolumn{8}{c}{Not a user-based evaluation: only a technical test performed.} \\
\cite{yun2018design} & Person carrier robot (wheelchair) & - & - & - & \textcolor{MyCrimson}{Heavy} & - & - & - & Bulky \\
\hline
\end{tabularx}
\end{table*}


==> texs/back-up/bck-t_prototype_information.tex <==
\begin{sidewaystable*}[t]
    % \begin{table*}
    % \footnotesize
     \scriptsize
    \centering
    \caption{\textbf{This table presents system prototype information. The Sensors and Computing resource used in the system prototype might differ from those listed in Table \ref{tab:core_technical_features}. This is because this table includes all sensors for the system prototype, not just those specific to the SLAM component.}}
    \label{tab:t_prototype_information}
    \setlength{\tabcolsep}{3pt}
    \begin{tabularx}{\textwidth}{p{20pt} p{30pt} X p{60pt} p{80pt} p{80pt} p{50pt} p{50pt} X }
    \hline
    \rowcolor{yellow}
    \textbf{Ref.} & \textbf{Carrying mode} & \textbf{Functionalities} & \textbf{Sensors} & \textbf{Computing resource} & \textbf{HCI} & \textbf{Assistive tool} & \textbf{Battery life} & \textbf{ML-based} \\
    \hline

    % 
    %  Part 1
    % 
    \cite{ahmetovic2023sonification} & Not mentioned & Navigation & Camera & Smartphone & \textcolor{blue}{Audio} & Smartphone &  &   \\
    \cite{li2022sensing} & Wearable & Navigation: positioning and wayfinding. Multi-target recognition: object localization, face recognition, and scene text recognition. & RGB-D camera, Ultrasonic sensor & Embedded computer, remote server & \textcolor{blue}{Audio}, \textcolor{teal}{haptic} & Electronic glasses and leg-mounted haptic modules & Over 12 hours under typical usage & Multi-target recognition \\
    \cite{song2023mixture} & Wearable & Real-time perception, remote assistance (leveraging WebRTC protocol), live broadcasts, chatrooms, real-time tagging & A depth, an RGB, and four gray scale cameras, an IMU & Microsoft Hololens2 device, GPU & \textcolor{blue}{Audio} & Microsoft Hololens2 &  &  \\
    \cite{zhang2023research} & \textcolor{blue}{Robot system} \textcolor{red}{check whay I put Handheld before} & Considerate navigation, spatial risk mapping, adaptive motion control & A 2D range sensor, 2 RGB-D RealSense D435 cameras & Two notebook PCs & \textcolor{blue}{Audio} & Wheeled guide mobile robot &  & Pedestrian detection (OpenPose), OpenCV ObjDetect Module Face Recognition, Yolact obstacle recognition, Speech recognition \\
    \cite{yang2022unav} & Wearable & Visual-based localization, location estimation, direction estimation, and navigation support & Phone’s camera & Cloud server and Nvidia Jetson AGX Xavier & \textcolor{blue}{Audio} & Android application &  & NetVLAD for global descriptors and SuperPoint for local descriptors to aid in the localization process \\
    \cite{zhou2022multi} & \textcolor{blue}{Robot system} & Localization & LiDAR, cameras & Nvidia Titan X GPU & No device & No device &  & GAN-based localization \\
    \cite{hou2022knowledge} & Wearable & Active navigation with sub-goal inference, context-aware Object Relation Prior Knowledge & RealSense D435i RGB-D camera & Jetson AGX Xavier & \textcolor{blue}{Audio} & Helmet; white cane for obstacle avoidance &  & An unbiased Scene Graph Generation (SGG) model to create scene graphs, then aggregates them into an Object Relation Knowledge Graph \\
    \cite{plikynas2022indoor} & Wearable & Scene description, face recognition, optical character recognition, obstacle recognition, social networking, remote assistance & IMU, stereo, IR (depth) camera & Raspberry Pi4, Cloud server & \textcolor{blue}{Audio}, \textcolor{violet}{tactile} & Smartphone &  & Faster RCNN: object detection, LSTM RNN: scene description, imitation-learning deep neural networks: navigation, Google Tensorflow im2txt: :scene captioning, Neurotechnology’s Verilook 12.2: face recognition \\
    \cite{xie2022multi} & \textcolor{violet}{Handheld} & Vibrations and sounds for obstacle avoidance, detailed mapping, real-time object recognition, and a smart cane for spatial orientation & RealSense RGB-D camera & Raspberry Pi & \textcolor{blue}{Audio}, \textcolor{violet}{tactile} & Smart cane &  & YOLO: Object detection \\
    \cite{qiu2022egocentric} & \multicolumn{7}{c}{No prototype implemented; the proposed approach for trajectory forecasting was tested with a robot.} & AlphaPose: to detect and track the nearby people appearing in each frame; PSPNet: to segment scene semantics; Monodepth2: to estimate depth from the monocular RGB frames; Transformer-based encoder-decoder neural network model: containing a novel cascaded cross-attention mechanism to fuse encodings of different modalities for trajectory forecasting. \\
    \cite{chen2021wearable} & Wearable & Real-time navigation, real-time semantic understanding, voice interaction, precise localization, real-time map generation & RGB-D camera & High-performance portable processor, cloud server & \textcolor{blue}{Audio} & A forehead mounted camera and an earphone to obtain the output information & & ENet for pixel-level semantic segmentation \\
    \cite{slade2021multimodal} & \textcolor{violet}{Handheld} & Obstacle avoidance, waypoint following, indoor/outdoor navigation, key object detection, user guidance through challenges & 2D LiDAR, camera, GPS antenna, IMU & A portable microcontroller & \textcolor{violet}{vibrotactile}, \textcolor{blue}{Audio}, Grounded kinesthetic & Augmented cane & Microcontroller: 4.2 and motor: 5.2 hours & YOLOV3Tiny for object detection, a linear regression model for distance estimation \\
    \cite{lu2021assistive} & \textcolor{blue}{Robot system} \textcolor{red}{ check why I put Handheld before} & UWB beacons for audio-based environmental information, dynamic obstacle avoidance, wall following, adjustable speed, and emergency stop. & Velodyne LiDAR VLP16, RealSense D345 depth camera & an Intel NUC computer, Nvidia Jetson TX2, Raspberry Pi3 & \textcolor{blue}{Audio}, \textcolor{teal}{haptic} & Guiding robot & & Reinforcement learning \\
    \cite{hakim2021indoor} & Wearable & Mapping, path planning, obstacle avoidance, transparent object detection, and path following. & RGB-D camdera (Asus Xtion Pro live), Ultrasonic sensor & Raspberry Pi3 B+ & \textcolor{blue}{Audio} & Head-mounted camera & & $\bullet$ \\
    \cite{zhang2021rgb} & \textcolor{violet}{Handheld} & Active steering for user guidance, obstacle avoidance, and wayfinding. & Realsense D435 (RGB-D) Camera, VN100 IMU & UP Board computer & \textcolor{blue}{Audio}, \textcolor{violet}{tactile} & Smart cane & & $\bullet$ \\
    \cite{cheng2021hierarchical} & Wearable & Obstacle avoidance, scene perception, and hierarchical localization services. & RealSense RGB-D-IR camera, IMU, a customized GNSS receiver & A portable computer, Nvidia Jetson TX2 & Not provided & Auxiliary glasses &  & NetVLAD and Dense Desc for advanced descriptor extraction. \\
    \cite{liu2020indoor} & \textcolor{violet}{Handheld} & Accurate object detection, semantic mapping, and indoor localization services. & hand-held RGB-D camera & Odroid XU3 board, remote server (data processing) & \textcolor{blue}{Audio} & No device & & ConvNet for semantic information extraction and location inference; Inception-v3 for object recognition. \\

    % 
    % part 2
    % 
    \cite{jin2020combining} & Wearable & Object detection and people detection for obstacle avoidance. & Two monocular cameras & Not mentioned & \textcolor{blue}{Audio} & Smart eyeglasses & Not mentioned & YOLOv2 for person detection. \\
    \cite{bai2019wearable} & Wearable & Obstacle avoidance, surrounding perception. & RGB-D camera, IMU, GPS & A smartphone with Qualcomm Snapdragon 820 CPU 2.0 GHz & \textcolor{blue}{Audio} & Eyeglasses-mounted sensors + smartphone & Not mentioned & PeleeNet + SDD for object recognition \\
    \cite{zhang2019arcore} & Wearable & Adaptive artificial potential field path planning and semantic understanding. & Smartphone's camera, Gravity sensor, Ambient light sensor, Proximity sensor, Gyroscope Compass & A HUAWEI P20 smartphone with Kirin 970 CPU & \textcolor{blue}{Audio}, \textcolor{teal}{haptic} & ARCore-supported smartphone + haptic gloves & Not mentioned & Not mentioned \\
    \cite{bai2018virtual} & Wearable & Locating, way-finding, route following, and obstacle detection. & Fisheye and depth camera, ultrasonic rangefinder & An embedded CPU board & \textcolor{blue}{Audio}, visual hints & Optical see-through glasses & Not mentioned & $\bullet$ \\
    \cite{zhang2017indoor} & \textcolor{violet}{Handheld} & Wayfinding 3D object detection & SwissRanger SR4000 3D camera & Client: HP Stream 7 tablet, server: Lenovo ThinkPad T430 laptop (Intel i5-3320M 2.6GHz CPU, NVS 5400m with 96 CUDA core) & \textcolor{blue}{Audio} & Smart cane & Not mentioned & $\bullet$ \\
    \cite{zhang2020plane} & \textcolor{violet}{Handheld} & Pose estimation, obstacle detection and avoidance, wayfinding & SwissRanger SR4000 camera, IMU (VN-100 of VectorNav Technolofgies) & Up Board computer & \textcolor{blue}{Audio} & Computer-vision-enhanced white cane & Not mentioned & $\bullet$ \\
    \cite{albogamy2021sravip} & \textcolor{blue}{Robot system} & Robot navigation, obstacle avoidance, path planning, and user interaction & Encoder, IMU, laser distance sensor, camera & Raspberry Pi 3 Model B and B+ & \textcolor{blue}{Audio} & Smart robot (Turtlebot3 robot)  & Not mentioned & $\bullet$ \\
    \cite{crabb2023lightweight} & \textcolor{violet}{Handheld} & Wayfinding and localization. & iPhone 11 Pro sensors & iPhone 11 Pro & Not mentioned & iPhone 11 Pro & Not mentioned & YOLOv2 for object detection to facilitate effective localization \\
    \cite{son2022wearable} & Wearable & Scene understanding, localization, object detection, path planning, path following, timely completion & Realseanse D435i RGB-D camera, compass sensor (BNO055 Bosch) & Jetson Xavier AGX, NVidia & \textcolor{blue}{Audio} & Head-worn camera & Not mentioned & Bisenet \& HarDNet for crosswalk, the end of the crosswalk (a red texture plate), and the crosswalk signal detection \\
    \cite{hakim2019indoor} & \textcolor{violet}{Handheld} & Safely navigate to destinations in static unfamiliar areas and identify surrounding objects. & Neato XV-11 LiDAR, ultrasonic sensor, Raspberry pi camera (CameraPi) & Raspberry Pi3 B+ & \textcolor{blue}{Audio} & Sensors attached to a white cane & Long battery life expected & Tiny YOLOv2 for predicting object class. \\
    \cite{goswami2023efficient} & No device & Real-time global localization & ZED2 RGB-D, IMU & Nvidia Jetson AGX Xavier microprocessor & No device & No device & Not mentioned & MobileNetV2 with PPM for constructing semantic point cloud \\
    \cite{hao2022detect} & Wearable & Detecting and locating objects of interest; guiding users efficiently to target objects. & Monocular camera & Nvidia Jetson Xavier NX Developer kit & \textcolor{blue}{Audio}, Virtual Touch \cite{liu2021virtual} & Chest-mounted camera & Not mentioned & Pretrained YOLOv5 for object detection \\
    \cite{kuribayashi2023pathfinder} & \textcolor{violet}{Handheld} & Intersection detection and sign recognition & 360\degree~LiDAR, iPhone 12 Pro camera & Nvidia RTX 3080 graphic board & \textcolor{blue}{Audio}, Handle interface & Suitcase-shaped robot & \textcolor{MyCrimson}{Low}: 2.6 hours & EasyOCR and YOLOv5 for sign recognition \\
    \cite{agrawal2022novel} & \textcolor{violet}{Handheld} & Finding socially preferred chairs & RGB-D from the RealSense D455 and IMU from the T265 cameras & Dell G15 laptop with an RTX 3060 GPU &  \textcolor{blue}{Audio}, \textcolor{teal}{haptic} & Robotic cane & - & Detectron2 for object detection and Mask-RCNN for obtaining masks for classiﬁcation. \\
    \cite{rui2021multi} & \textcolor{violet}{Handheld} & Multi-sensory guidance, obstacle avoidance, real-time target detection & RBG-D camera & Uzel US-M5422 edge server, Raspberry Pi 4B & \textcolor{blue}{Audio}, \textcolor{violet}{tactile} & Smart cane & Not mentioned & YOLO for target detection \\
    \cite{ou2022indoor} & Wearable & Localization and mapping in dynamic environments, obstacle avoidance, dynamic object tracking. & RGB-D camera & Laptop & \textcolor{blue}{Audio} & Smart glasses & Not mentioned & PanopticFCN for obtaining the prior dynamic object information, OpenPose for obtaining a more accurate speed estimation of dynamic moving people \\

    % 
    % part 3
    % 
    \cite{jin2021wearable} & Wearable & Locating a target object, wayfinding, motion guidance, and grasping the object. & Occipital-Structure Core sensor with a built-in Bosch BMI055 IMU, a color camera, and a global shutter stereo IR camera & Google Pixel 3 smartphone equipped with a Snapdragon 845 processor and 4 GB RAM. & \textcolor{blue}{Audio}, \textcolor{teal}{haptic} & Hand-worn device & Not mentioned & TensorFlow Lite Object Detection API (MobileNet SSD model) for detecting the target object \\
    \cite{xu2021multi} & Wearable & Indoor navigation, real-time path planning, object of interest detection & RealSense D435i camera & Embeded Jetson nano 4GB, remote server based on Intel i7-8700 CPU, nvidia GTX1080 GPU, 64 GB DDR4 RAM & \textcolor{blue}{Audio}, \textcolor{teal}{haptic} & Smart E-glasses & Over 12 hours per charge & MobilenetV3-Yolov4-Lite, based on YOLOv4 and MobileNetV3 for object detection \\
    \cite{lu2021personalized} & Wearable & Detecting and describing objects in environments, personalizing navigation through interactive dialogues and re-training, and locating users. & Google glasses camera & GPU server & Not mentioned & Google glasses & Not mentioned & YOLOv4 and SSD for detecting and describe objects, a classical attention-based encoder-decoder model with LSTM and ResNet \cite{xu2015neural} for image captioning. \\
    \cite{kayukawa2020guiding} & \textcolor{violet}{Handheld} & Collision risk prediction, directional guidance, mode switching, obstacle avoidance, real-time feedback. & Two RealSense D435 RGB-D cameras, IMU, LiDAR & Laptop (Intel Core i7-8750H CPU @ 2.20GHz, NVIDIA GeForce GTX 1080 Mobile GPU) & \textcolor{blue}{Audio}, \textcolor{violet}{tactile} & A rolling suitcase-shaped device & Not mentioned & YOLOv3 for detecting surrounding pedestrians. \\
    \cite{chen2020navigation} & No device & Route planning and obstacle avoidance. & RGB-D camera, IMU, LiDAR & Not mentioned & \textcolor{blue}{Audio} & No device & Not mentioned & Not mentioned \\
    \cite{chen2020can} & Wearable & Scene perception, obstacle avoidance, and localization & RealSense R200 camera & Nvidia Jetson AGX Xavier processor & \textcolor{blue}{Audio} & Smart glasses & Not mentioned & RFNet for generating semantic labels \\
    \cite{fusco2020indoor} & Either \textcolor{violet}{Handheld} or wearable & Real-time localization and turn-by-turn directions. & iPhone 8's IMU and rear-facing camera & iPhone 8 & \textcolor{blue}{Audio} & Smartphone & \textcolor{MyCrimson}{Low}: 13\% usage in 16 minutes. & Not explicitly mentioned \\
    \cite{zhang2019human} & \textcolor{violet}{Handheld} & Wayfinding, human intent detection, and human-robot interaction & RealSense D435 Camera, IMU (VN100 of VectorNav Technologies, LLC) & UP Board computer & \textcolor{blue}{Audio}, motorized rolling tip & White-cane mounted camera & Not mentioned & $\bullet$ \\
    \cite{zhao2019multi} & Wearable & Semantic mapping and path planning, obstacle avoidance, environment perception & RPLIDAR A2, Microsoft Kinect VI, ZED stereo camera  & Laptop & \textcolor{blue}{Audio} & TurtleBot2 robot (to be replaced by portable device) + wearable sensors & Not mentioned & YOLOv3 for landmark detection, Places365 for place recognition \\
    \cite{weiss2020navigation} & \multicolumn{8}{c}{Paper develops a Reinforcement Learning environment to create a navigation assistant tailored for the BVI community, without prototype implementation.}  \\
    \cite{ramesh2018real} & \textcolor{violet}{Handheld} & Real-time localization, navigation, object detection, and distance-depth estimation, using a single monocular camera. & Monocular camera & Intel i7 processor & \textcolor{blue}{Audio}  & Smartphone & Not mentioned & ACF detector for object detection to identify trained objects of interest for localization. \\
    \cite{eden2018indoor} & No device & Enhanced indoor localization and navigation using environmental texts. & Smartphone and ZED cameras & Nvidia Jetson TX2 & No device & No device & No device & CNN or text detection and recognition \\
    \cite{mulky2018autonomous} & Ride-on & Autonomous navigation, real-time mapping and localization, obstacle avoidance, accurate steering. & IMU, MPU-9250, stereo camera, laser, LiDAR & Nvidia Jetson TX2, Raspberry Pi, and Arduino. & Steering control & Intelligent autonomous scooter & Not mentioned & $\bullet$ \\
    \cite{lalonde2018localizing} & Wearable & Tracking blind pedestrians' paths & Hero3+ GoPro & Not mentioned & Not mentioned & Wearable camera & Not mentioned & $\bullet$ \\
    \cite{zhang2017plane} & \textcolor{violet}{Handheld} & Pose estimation, wayfinding assistance & Time-of-flight camera (SwissRanger SR4000), IMU (VN 100 of VectorNav Technologies, LLC) & UP Board computer & Not mentioned & Computer-vision-enhanced white cane & Not mentioned & $\bullet$ \\

    %
    % part 4
    %
    
    \cite{chen2017ccny} & \textcolor{violet}{Handheld} & Indoor mapping, path planning, control panel interface, and object avoidance. & Wide-angle lens camera, gyroscope, accelerometers, and infrared sensor on Google Tango, IMU on the cane. & Google Tango, microcontroller & \textcolor{blue}{Audio}, \textcolor{teal}{haptic} & Smart cane + Google Tango & Lasts approximately 17 hours & $\bullet$ \\
    \cite{bai2017cloud} & Wearable & Obstacle avoidance, OCR, path planning, and human assistance via web application. & Stereo camera & Cloud server & \textcolor{blue}{Audio} & Helmet-mounted camera + android-based smartphone & Not mentioned & Recurrent Convolutional Neural for object detection and recognition, \cite{farabet2012learning, noh2015learning} for scene parsing, \cite{neumann2015real, akbani2015character} for Optical Character Recognition, \cite{shao2010paper} for currency recognition, and \cite{weber2016deeptlr} for traffic light recognition \\
    \cite{endo2017indoor} & Wearable & Route guidance to a destination, obstacle avoidance & Monocular camera & A single CPU & Not mentioned & Wearable camera & Not mentioned & $\bullet$ \\
    \cite{yang2022seeway} & \textcolor{violet}{Handheld} & Global path finding, local path re-planning, and obstacle avoidance. & Camera, IMU, inbuilt 3D LiDAR from iPhone 12 Pro Max & Smartphone, AWS Lambda on cloud & \textcolor{blue}{Audio} & iPhone 12 Pro Max & Not mentioned & SFSpeechRecognizer from iOS for speech-to-text, ResNet for extracting feature representation of each viewpoint for scene-graph map construction, EnvDrop for path exploration, and reinforcement learning for training the Vision-Language Navigation agent to navigate indoor environments based on language instructions. \\
    \cite{shahani2023methods} & Wearable & Wayfinding and identifying short-term impediments with GeoNotify smartphone software. & Kinect camera & Not mentioned & \textcolor{blue}{Audio}, \textcolor{teal}{haptic} & Wearable camera & Not mentioned & YOLOv4 Tiny for object detection \\
    \cite{yun2018design} & Ride-on & Navigation, path following, obstacle avoidance. & Hokuyo's URG-04LX-UG01 Laser Range Finder (LRF) sensor, Microsoft LifeCam HD-5000 USB camera, MTi-30 Attitude Heading Reference System (AHRS) IMU sensor from Xsens & PC & Autonomous navigation & Person carrier robot (wheelchair) & Not mentioned & $\bullet$ \\
    \hline
    \end{tabularx}
    % \end{table*}
\end{sidewaystable*}

==> texs/back-up/bck-t_user_evaluation.tex <==
\begin{table*}[t]
    \centering
    \caption{User Evaluation. Some studies only mentioned the number of participants in the experiments, without specifying their visual abilities. In such cases, column "\# Participants" indicates "AU" to denote that the abilities are unspecified. NM indicates that specific information was not mentioned in the literature.}
    \label{tab:t_user_evaluation}
    \setlength{\tabcolsep}{3pt}
    \begin{tabularx}{\textwidth}{ p{20pt} >{\centering\arraybackslash}p{25pt} >{\centering\arraybackslash}p{35pt} >{\centering\arraybackslash}p{35pt} >{\centering\arraybackslash}p{30pt} >{\centering\arraybackslash}p{20pt} X X }
    \hline
    \rowcolor{yellow}
    \multirow{2}{*}{\textbf{Ref.}} & \multicolumn{2}{c}{\textbf{\# Participants}} & \multicolumn{3}{c}{\textbf{Method of evaluation}} & \multirow{2}{*}{\textbf{Experimental site}} & \multirow{2}{*}{\textbf{User satisfaction}} \\
    \cline{2-3}
    \cline{4-6}
     & \textbf{BVI} & \textbf{Blindfolded} & \textbf{User study} & \textbf{Interview} & \textbf{Survey} & & \\
    \hline

    % 
    % part 1
    % 
    
    \cite{ahmetovic2023sonification} & 9 & 0 & $\checkmark$ & $\bullet$ & $\checkmark$ & A university campus & Participants' feedback varied on pleasantness, annoyance, precision, quickness, and overall appreciation of sonification. \\
    \cite{li2022sensing} & 2 & 3 & $\checkmark$ & $\bullet$ & $\bullet$ & Wearable Robotics and Autonomous Unmanned Systems Laboratory at the University of Science and Technology of China & No overall satisfaction score; details on task success rates, completion times, and verbal/haptic feedback.\\
    \cite{song2023mixture} & 5 & 3 & $\checkmark$ & $\bullet$ & $\bullet$ & Not mentioned & Scores 6-9 out of 10 \\
    \cite{zhang2023research} & 0 & 10 & $\checkmark$ & $\bullet$ & $\checkmark$ & Not mentioned & Moderate: improved acceptance and trust levels noted \\
    \cite{yang2022unav} & 2 & 4 & $\checkmark$ & $\bullet$ & $\bullet$ & New York University Langone Ambulatory Care Center (A Complex hospital environmnet) & Not mentioned \\
    \cite{zhou2022multi} & 0 & 0 & $\bullet$ & $\bullet$ & $\bullet$ & The corridor environment of a typical ofﬁce building & Not a user-based evaluation (a technical test) \\
    \cite{hou2022knowledge} & 0 & 8 & $\checkmark$ & $\checkmark$ & $\bullet$ & A room & Moderate to high satisfaction: Users found the system acceptable and useful for indoor navigation \\
    \cite{plikynas2022indoor} &  78 & 0 & $\bullet$ & $\bullet$ & $\checkmark$ & Surveyed BVI online using LymeSurvey to understand social networking needs & Not mentioned; the focus is on system development \\
    \cite{xie2022multi} & 0 & 1 & $\checkmark$ & $\bullet$ & $\bullet$ & A laundry room, H-shaped hallway, classroom, and T-shaped hallway & Not mentioned; the focus is on system development \\
    \cite{qiu2022egocentric} & 0 & 0 & $\bullet$ & $\bullet$ & $\bullet$ & \multicolumn{2}{c}{Not a user-based evaluation (a technical test)} \\
    \cite{chen2021wearable} & \multicolumn{7}{c}{Not explicitly mentioned; the focus is on a technical test.} \\
    \cite{slade2021multimodal} & 12 & 12 & $\checkmark$ & $\bullet$ & $\checkmark$ & Hallways constructed with cardboard, outdoor & Novice and expert users noted usability challenges due to weight, but confidence and workload improved \\
    \cite{lu2021assistive} & 8 & 0 & $\checkmark$ & $\checkmark$ & $\checkmark$ & A hallway in the Boai Campus BIO–ICT Building on the campus of National Yang Ming Chiao Tung University, Taiwan & Participants found the proposed route easy to navigate, with low perceived difficulty and medium confidence. Most intend to use it again. \\
    \cite{hakim2021indoor} & \multicolumn{5}{c}{Not explicitly mentioned} & Laboratory & Not mentioned \\
    \cite{zhang2021rgb} & \multicolumn{5}{c}{The focus is on a technical test} & The Engineering East Hall of Virginia Commonwealth University & Technical focus only \\
    \cite{cheng2021hierarchical} & \multicolumn{7}{c}{Focuses on technical performance; real-world user satisfaction not directly assessed.} \\
    \cite{liu2020indoor} & \multicolumn{7}{c}{The technical test was conducted in accommodation and office buildings. Real-world user satisfaction was not directly assessed.} \\
    \cite{jin2020combining} & \multicolumn{7}{c}{The technical test was conducted in a university lobby. Real-world user satisfaction was not directly assessed.} \\
    \cite{bai2019wearable} & 20 & 0 & $\checkmark$ & $\bullet$ & $\checkmark$ & Office area and simulated outdoor scenario & Positive feedback on usability and navigation; desire for detailed tutorials; satisfaction with daily use, challenges with multi-floor navigation. \\
    \cite{zhang2019arcore} & 4 & 0 & $\checkmark$ & $\bullet$ & $\checkmark$ & In a corridor & All subjects found haptic instructions intuitive, enhancing safety and reducing hesitation compared to audio, though some suggested design improvements. \\
    \cite{bai2018virtual} & Unspecified & 0 & $\checkmark$ & $\bullet$ & $\bullet$ & Not mentioned & Not mentioned \\
    \cite{zhang2017indoor} & 0 & 7 & $\checkmark$ & $\bullet$ & $\checkmark$ & Various indoor places & Users find the wayfinding function useful, but discomfort due to weight is a significant concern. \\
    \cite{zhang2020plane} & \multicolumn{7}{c}{The technical test was conducted on seven datasets collected internally. Real-world user satisfaction was not directly assessed.} \\
    \cite{albogamy2021sravip} & \multicolumn{7}{c}{The test was conducted in the College of Computer and Information Sciences at King Saud University, but user satisfaction was not directly assessed.} \\
    \cite{crabb2023lightweight} & 1 & 5 & \multicolumn{5}{c}{Data was collected by participants to simulate indoor navigation, followed by offline analysis. User satisfaction was not assessed.} \\
    \cite{son2022wearable} & 3 & 0 & $\checkmark$ & $\checkmark$ & $\bullet$ & Two different crosswalks & Intuitive, easy-to-understand verbal instructions, enhances street crossing safety \\
    \cite{hakim2019indoor} & \multicolumn{7}{c}{The technical test was conducted in various indoor environments. Real-world user satisfaction was not directly assessed.} \\
    \cite{goswami2023efficient} & \multicolumn{7}{c}{The technical test was conducted in a corridor environment. Real-world user satisfaction was not directly assessed.} \\
    \cite{hao2022detect} & \multicolumn{7}{c}{The technical test was conducted in an office room and on the KITTI dataset. Real-world user satisfaction was not directly assessed.} \\
    \cite{kuribayashi2023pathfinder} & 7 & 0 & $\checkmark$ & $\checkmark$ & $\bullet$ & In unfamiliar building & High satisfaction with PathFinder's navigation assistance, intersection detection, and audio feedback. \\
    \cite{agrawal2022novel} & 0 & 6 & $\checkmark$ & $\bullet$ & $\checkmark$ & In a conﬁgurable 12ft × 17ft room & High confidence, ease of use, and performance rated positively; verbal overview and haptics well-received for navigation assistance. \\
    \cite{rui2021multi} & \multicolumn{7}{c}{The technical test was conducted on the KITTI-02 dataset. Real-world user satisfaction was not directly assessed.} \\
    \cite{ou2022indoor} & \multicolumn{7}{c}{The technical test included TUM RGB-D, Bonn RGB-D datasets, and real-life sequences, but didn't directly assess user satisfaction.} \\
    \cite{jin2021wearable} & 0 & 5 & $\checkmark$ & $\bullet$ & $\bullet$ & In a laboratory & The significant improvement in success rate and task completion time, from 32\% to 96\% and 29.1s to 15.6s respectively, demonstrates the effectiveness of the proposed solution in aiding wayfinding and object manipulation. \\

    % 
    % part 2
    % 
    
    \cite{xu2021multi} & \multicolumn{2}{c}{3; AU} & $\checkmark$ & $\bullet$ & $\bullet$ & Not explicitly mentioned & User satisfaction not directly assessed; technical tests show high success rates and accuracy. \\
    \cite{lu2021personalized} & \multicolumn{2}{c}{1; AU} & $\checkmark$ & $\bullet$ & $\bullet$ & In a laboratory & User satisfaction not assessed \\
    \cite{kayukawa2020guiding} & 14 & 0 & $\checkmark$ & $\bullet$ & $\checkmark$ & A short route in a controlled and long route in a real-world public space. & Participants expressed high levels of contentment with the system's usability, effectiveness, and overall user experience in the study. \\
    \cite{chen2020navigation} & \multicolumn{7}{c}{Initiating target user testing was not feasible as the system was in the experimental stage.} \\
    \cite{chen2020can} & 0 & 1 & $\checkmark$ & $\bullet$ & $\bullet$ & Not mentioned & Assessed through successful task completion, yet occasional false positives slightly affect confidence. \\
    \cite{fusco2020indoor} & 5 & 0 & $\checkmark$ & $\bullet$ & $\bullet$ & Smith-Kettlewell building & Not mentioned \\
    \cite{zhang2019human} & \multicolumn{7}{c}{The technical test was conducted in the East Engineering Building at VCU. Real-world user satisfaction was not directly assessed.} \\
    \cite{zhao2019multi} & 0 & 1 & $\checkmark$ & $\bullet$ &$\bullet$ & In a laboratory & The technical test was conducted. Real-world user satisfaction was not directly assessed. \\
    \cite{weiss2020navigation} & \multicolumn{7}{c}{Paper develops a Reinforcement Learning environment to create a navigation assistant tailored for the BVI, without user-based evaluation.}\\
    \cite{ramesh2018real} & \multicolumn{7}{c}{Technical tests conducted on the Karlsruhe dataset, indoor recorded dataset, and in a house; user satisfaction not assessed.} \\
    \cite{eden2018indoor} & \multicolumn{7}{c}{Technical tests conducted in a research building; user satisfaction not assessed.} \\
    \cite{mulky2018autonomous} & \multicolumn{7}{c}{Not explicitly mentioned; the focus is on a technical test.} \\
    \cite{lalonde2018localizing} & \multicolumn{2}{c}{1; AU}& \multicolumn{5}{c}{Not explicitly mentioned; the focus is on a technical test.} \\
    \cite{zhang2017plane} & \multicolumn{7}{c}{The technical test was conducted on seven datasets collected in two buildings. Real-world user satisfaction was not directly assessed.} \\
    \cite{chen2017ccny} & 0 & Number unspecified & $\checkmark$ & $\bullet$ & $\bullet$ & In various indoor environments (university campus, hotel, office building) & Not assessed \\
    \cite{bai2017cloud} & \multicolumn{7}{c}{The technical test was conducted in an office and pedestrian street. Real-world user satisfaction was not directly assessed.} \\
    \cite{endo2017indoor} & \multicolumn{7}{c}{The technical test was conducted in a laboratory. Real-world user satisfaction was not directly assessed.} \\
    \cite{yang2022seeway} & 10 & 1 & By a sighted user & Conducted with 10 BVI & $\bullet$ & In the Rhodes Research Center at Clemson University & An online interview with 10 BVI individuals via Zoom guided the choice of a 3D perception-enabled mobile platform with a speech-auditory interface. Real-world user satisfaction was not directly assessed.% Technical tests on Matterport3D and Clemson-VLN datasets evaluated global path generation quantitatively and qualitatively. 
    \\
    \cite{shahani2023methods} & \multicolumn{7}{c}{ Real-world user satisfaction was not directly assessed.} \\
    \cite{yun2018design} & \multicolumn{7}{c}{Technical tests conducted in a corridor; user satisfaction not assessed.} \\
    \hline
    \end{tabularx}
\end{table*}


==> texs/back-up/paper_title.tex <==
ahmetovic2023sonification [56] Sonification of navigation instructions for people with visual
li2022sensing [57] Sensing and Navigation of Wearable Assistance Cognitive
song2023mixture [58] Mixture reality-based assistive system for visually impaired
zhang2023research [59] Research on Design and Motion Control of a Considerate
yang2022unav [60] UNav: An Infrastructure-Independent Vision-Based Navigation System for People with Blindness and Low Vision
zhou2022multi [61] Multi-Floor Indoor Localization Based on Multi-Modal Sensors
hou2022knowledge [62] Knowledge driven indoor object-goal navigation aid for visually impaired people
plikynas2022indoor [63] Indoor-Guided Navigation for People Who Are Blind:
xie2022multi [64] A Multi-Sensory Guidance System for the Visually Impaired
qiu2022egocentric [65] Egocentric Human Trajectory Forecasting with a Wearable
chen2021wearable [66] A wearable navigation device for visually impaired people
slade2021multimodal [67] Multimodal sensing and intuitive steering assistance improve navigation and mobility for people with impaired
lu2021assistive [68] Assistive Navigation Using Deep Reinforcement Learning
hakim2021indoor [69] Indoor Wearable Navigation System Using 2D SLAM Based
zhang2021rgb [70] An RGB-D Camera Based Visual Positioning System for
cheng2021hierarchical [71] Hierarchical visual localization for visually impaired people
liu2020indoor [72] Indoor Topological Localization Based on a Novel Deep
jin2020combining [73] Combining Obstacle Avoidance and Visual Simultaneous
bai2019wearable [74] Wearable travel aid for environment perception and navigation of visually impaired people
zhang2019arcore [75] An ARCore based user centric assistive navigation system
bai2018virtual [76] Virtual-Blind-Road Following-Based Wearable Navigation
zhang2017indoor [77] An indoor wayfinding system based on geometric features
zhang2020plane [78] Plane-Aided Visual-Inertial Odometry for 6-DOF Pose Estimation of a Robotic Navigation Aid
albogamy2021sravip [79] SRAVIP: Smart Robot Assistant for Visually Impaired Persons
crabb2023lightweight [80] A Lightweight Approach to Localization for Blind and Visually Impaired Travelers
son2022wearable [82] Wearable system to guide crosswalk navigation for people
hakim2019indoor [83] Indoor Low Cost Assistive Device using 2D SLAM Based
goswami2023efficient [84] Efficient Real-Time Localization in Prior Indoor
hao2022detect [85] Detect and Approach: Close-Range Navigation Support for People with Blindness and Low Vision
kuribayashi2023pathfinder [87] PathFinder: Designing a Map-Less Navigation System for Blind People in Unfamiliar Buildings
agrawal2022novel [88] A Novel Perceptive Robotic Cane with Haptic Navigation for Enabling Vision-Independent Participation in the Social Dynamics of Seat Choice
rui2021multi [89] A Multi-Sensory Blind Guidance System Based on
ou2022indoor [90] Indoor Navigation Assistance for Visually Impaired
jin2021wearable [91] A Wearable Robotic Device for Assistive Navigation
xu2021multi [92] Multi-functional smart E-glasses for vision-based indoor navigation
lu2021personalized [93] Personalized Navigation that Links Speaker’s Ambiguous Descriptions to Indoor Objects for Low Vision People
kayukawa2020guiding [95] Guiding Blind Pedestrians in Public Spaces by Understanding Walking Behavior of Nearby Pedestrians
chen2020navigation [96] A Navigation Aid for Blind People Based on Visual
chen2020can [97] Can we unify perception and localization in assisted
fusco2020indoor [98] Indoor Localization for Visually Impaired Travelers
zhang2019human [99] Human-Robot Interaction for Assisted Wayfinding
zhao2019multi [100] A Multi-Sensor Fusion System for Improving Indoor
weiss2020navigation [101] Navigation Agents for the Visually Impaired: A Sidewalk Simulator and Experiments
ramesh2018real [102] Real-time localization and navigation in an indoor
eden2018indoor [103] Indoor Navigation using Text Extraction Eden, Jake and Kawchak, Thomas and Narayanan, Vijaykrishnan
mulky2018autonomous [104] Autonomous Scooter Navigation for People with Mobility
lalonde2018localizing [105] Localizing people in crosswalks using visual odometry: Preliminary results
zhang2017plane [106] Plane-aided visual-inertial odometry for pose estimation of
chen2017ccny [107] CCNY Smart Cane Chen, Qingtian and Khan, Muhammad and Tsangouri,
bai2017cloud [108] A Cloud and Vision-Based Navigation System Used for
endo2017indoor [109] Indoor positioning and obstacle detection for visually impaired navigation system based on LSD-SLAM
yang2022seeway [110] SeeWay: Vision-Language Assistive Navigation for the Visually Impaired
shahani2023methods [111] The Methods of Visually Impaired Navigating and Obstacle
yun2018design [112] The Design of Person Carrier Robot using SLAM and Robust Salient Detection

=======================================================================================

Sonification of navigation instructions for people with visual impairment
Sensing and Navigation of Wearable Assistance Cognitive Systems for the Visually Impaired
Mixture reality-based assistive system for visually impaired people
Research on Design and Motion Control of a Considerate Guide Mobile Robot for Visually Impaired People
UNav: An Infrastructure-Independent Vision-Based Navigation System for People with Blindness and Low Vision
Multi-Floor Indoor Localization Based on Multi-Modal Sensors
Knowledge-driven indoor object-goal navigation aid for visually impaired people
Indoor-guided navigation for people who are blind: Crowdsourcing for route mapping and assistance
A multi-sensory guidance system for the visually impaired using YOLO and ORB-SLAM
Egocentric human trajectory forecasting with a wearable camera and multi-modal fusion
A wearable navigation device for visually impaired people based on the real-time semantic visual SLAM system
Multimodal sensing and intuitive steering assistance improve navigation and mobility for people with impaired vision
Assistive navigation using deep reinforcement learning guiding robot with UWB/voice beacons and semantic feedbacks for blind and visually impaired people
Indoor Wearable Navigation System Using 2D SLAM Based on RGB-D Camera for Visually Impaired People
An RGB-D Camera Based Visual Positioning System for Assistive Navigation by a Robotic Navigation Aid
Hierarchical visual localization for visually impaired people using multimodal images
Indoor topological localization based on a novel deep learning technique
Combining obstacle avoidance and visual simultaneous localization and mapping for indoor navigation
Wearable travel aid for environment perception and navigation of visually impaired people
An ARCore based user centric assistive navigation system for visually impaired people
Virtual-blind-road following-based wearable navigation device for blind people
An indoor wayfinding system based on geometric features aided graph SLAM for the visually impaired
Plane-aided visual-inertial odometry for 6-DOF pose estimation of a robotic navigation aid
SRAVIP: Smart Robot Assistant for Visually Impaired Persons
A Lightweight Approach to Localization for Blind and Visually Impaired Travelers
Appearance-based indoor place recognition for localization of the visually impaired person
Wearable System to Guide Crosswalk Navigation for People With Visual Impairment
Indoor Low Cost Assistive Device using 2D SLAM Based on LiDAR for Visually Impaired People
Efficient Real-Time Localization in Prior Indoor Maps Using Semantic SLAM
Detect and Approach: Close-Range Navigation Support for People with Blindness and Low Vision
3DMovieMap: an Interactive Route Viewer for Multi-Level Buildings
PathFinder: Designing a Map-less Navigation System for Blind People in Unfamiliar Buildings
A novel perceptive robotic cane with haptic navigation for enabling vision-independent participation in the social dynamics of seat choice
A multi-sensory blind guidance system based on YOLO and ORB-SLAM
Indoor Navigation Assistance for Visually Impaired People via Dynamic SLAM and Panoptic Segmentation with an RGB-D Sensor
A Wearable Robotic Device for Assistive Navigation and Object Manipulation
Multi-functional Smart E-Glasses for Vision-Based Indoor Navigation
Personalized Navigation that Links Speaker’s Ambiguous Descriptions to Indoor Objects for Low Vision People
Guiding Blind Pedestrians in Public Spaces by Understanding Walking Behavior of Nearby Pedestrians
A Navigation Aid for Blind People Based on Visual Simultaneous Localization and Mapping
Can We Unify Perception and Localization in Assisted Navigation? An Indoor Semantic Visual Positioning System for Visually Impaired People
Indoor Localization for Visually Impaired Travelers Using Computer Vision on a Smartphone
Human-Robot Interaction for Assisted Wayfinding of a Robotic Navigation Aid for the Blind
A Multi-Sensor Fusion System for Improving Indoor Mobility of the Visually Impaired
Navigation Agents for the Visually Impaired: A Sidewalk Simulator and Experiments
Real-time Localization and Navigation in an Indoor Environment Using Monocular Camera for Visually Impaired
Indoor Navigation Using Text Extraction
Autonomous Scooter Navigation for People with Mobility Challenges
Localizing People in Crosswalks using Visual Odometry: Preliminary Results
Plane-aided visual-inertial odometry for pose estimation of a 3D camera based indoor blind navigation
CCNY smart cane
A cloud and vision-based navigation system used for blind people
Indoor positioning and obstacle detection for visually impaired navigation system based on LSD-SLAM
SeeWay: Vision-Language Assistive Navigation for the Visually Impaired
The Methods of Visually Impaired Navigating and Obstacle Avoidance
The Design of Person Carrier Robot using SLAM and Robust Salient Detection

==> texs/draft/additions.tex <==



==> texs/draft/draft_03_results.tex <==
%
% Section 3: Result
\section{Result}
\label{results}
In this section, the findings of SLR are presented. Figure \ref{distribution_of_papers} shows the number of studies included in this review that focused on BVI navigation using SLAM techniques. As shown in the figure, although only papers published in the first half of 2023 are included in this review, they constitute a substantial portion of the total. The growth in the number of studies in this domain suggests an advancement in SLAM techniques and an increase in their usage for developing navigation technologies for visually impaired individuals. 
This section is divided into four parts to answer the research questions. It discusses the types of SLAM techniques used to develop assistive technologies for visually impaired navigation, delves into the advantages and limitations of these techniques, highlights the challenging scenarios addressed, and presents the attributes of SLAM-based solutions that contribute to the enhancement of visually impaired navigation.

% Figure 5. Publications included in this review on SLAM-based BVI navigation, by year
\begin{figure}
    \centering
    \includegraphics[scale=0.4]{images/05_distribution_of_papers.png}
    \caption{\textbf{Publications included in this review on SLAM-based BVI navigation, by year}}
    \label{distribution_of_papers}
\end{figure}

%
% RQ1
%
\subsection{RQ1. What localization and mapping approaches are used for the navigation of the visually impaired?}
Since there are many different types of SLAMs designed with different types of sensors, for different applications, and for different scenarios, in this section, we focus on reviewing the types of SLAM that have been used for navigation of visually impaired people. It is a key technology in robotics and computer vision and has the potential to assist visually impaired individuals with navigation. This can help visually impaired people by providing real-time maps and spatial awareness. Among the 57 papers surveyed, three strategies were common, as shown in Table \ref{rq1_slam_type}. In this table, we use the exact terms mentioned in the literature for the localization and mapping techniques. Most studies have incorporated widely applicable SLAM techniques, such as ORB-SLAM, and some have developed new solutions tailored to their needs. For example, \cite{jin2020combining} proposed visual simultaneous localization and mapping for the moving-person tracking (VSLAMMPT) method. The proposed method was designed to assist people with disabilities, particularly visually impaired individuals, in navigating indoor environments. Several studies have used the SLAM components of existing frameworks, such as ARCore and ZED camera SLAM.
The reviewed studies demonstrate the versatility of SLAM in various navigation scenarios. The specific implementation and aspects addressed in each study varied depending on the application. SLAM can be employed in environments that lack a map and can dynamically create it while navigating. This involves simultaneous map creation and localization within an environment, without a predefined map. In this scenario, SLAM simultaneously constructs a map of the environment and determines the location of an agent on the map. Alternatively, SLAM can be employed to generate maps for subsequent navigation. In this case, SLAM first builds a map of the environment and then the map is utilized during navigation. Studies have also used SLAM odometry for navigational tracking. Odometry provides a continuous estimate of the position and orientation of an agent based on the sensor readings.


% Table 10. RQ1. Localization and mapping approaches used for visually impaired navigation
\input{texs/tables/t10_RQ1_SLAM_type}

As Table \ref{rq1_slam_type} shows, most studies used visual sensor-based SLAM techniques. Advances in computer vision, image processing, and machine learning have significantly enhanced the capabilities of visual sensors in navigation tasks. SLAM algorithms can exploit these advancements to provide highly accurate and robust navigational solutions. Moreover, visual sensors provide a wealth of information regarding the environment, including objects, obstacles, landmarks, and navigation cues. This information can be used to create accurate maps, detect obstacles, and aid in navigation. Visual sensors are highly versatile and can function both indoors and outdoors. Cameras are also relatively affordable and do not significantly increase the cost of the overall device or system, making them a cost-effective choice for assistive technology.

Figure \ref{SLAM_over_time} provides insight into the use of various SLAM techniques for visually impaired navigation from 2017 to the date this SLR was conducted (July 2023). This figure illustrates that VSLAM has been consistently used across all years. Although many other techniques also operate based on visual data, we mentioned each of these techniques, as indicated in the referenced studies. 

The utilization of semantic SLAM and Cartographer SLAM signifies a recent trend towards leveraging advanced spatial understanding and mapping capabilities for visually impaired navigation. Semantic SLAM incorporates higher-level scene interpretation and enhances users’ contextual awareness. On the other hand, Cartographer SLAM provides SLAM in 2D and 3D across various platforms and sensor configurations, offering innovative solutions to tackle the diverse challenges associated with BVI navigation.

ORB-SLAM algorithms, including ORB-SLAM (published in 2015), ORB-SLAM2 (published in 2017), and ORB-SLAM3 (published in 2021), have gained popularity because of their robustness and performance. This can be attributed to its efficient feature extraction and matching techniques, making it well suited for real-time navigation applications.

Customized techniques were developed to meet specific needs. This trend indicates that researchers have adjusted the SLAM techniques to better match the specific requirements of their intended applications. This suggests closer integration of SLAM with domain-specific needs.

 % Fig. 6. Evolution and adoption of SLAM techniques in BVI navigation systems over time.
\begin{figure*}
    \centering
    \includegraphics[scale=.5]{images/06_SLAM_over_time.png}
    \caption{\textbf{Evolution and adoption of SLAM techniques in BVI navigation systems over time.}}
    \label{SLAM_over_time}
\end{figure*}

One of the key features of SLAM techniques is their adaptability to both indoor and outdoor environments. In indoor settings, where GPS signals may be unreliable or unavailable, SLAM is a crucial tool for localization and mapping. Of the 57 studies considered, 41 specifically employed SLAM for indoor navigation, highlighting its importance in addressing indoor positioning challenges. Four studies demonstrated the application of SLAM in outdoor scenarios. Additionally, five papers demonstrated the versatility of SLAM by using it for both indoor and outdoor navigation contexts, underscoring its adaptability across environments. Although seven studies did not explicitly specify the environmental context, the majority focused on indoor navigation, reflecting the significant role that SLAM plays in enhancing navigation capabilities within enclosed spaces. 
% Figure \ref{SLAM_usage_in_envirinmnets} provides a clear visual representation of the proportion of studies that used SLAM in indoor, outdoor, and mixed indoor-outdoor navigation contexts. 

% Fig. 7. SLAM usage in different navigation environments
% \begin{figure}
%     \centering
%     \includegraphics[scale=0.4]{images/07_SLAM_usage_in_envirinmnets.png}
%     \caption{\textbf{SLAM usage in different navigation environments.}}
%     \label{SLAM_usage_in_envirinmnets}
% \end{figure}

% 
% RQ2
%
\subsection{RQ2. What are the advantages and limitations of SLAM techniques for BVI navigation?}

%
% Advantages
%
\subsubsection{Advantages}
Unlike many localization approaches, such as RFID- or GPS-based methods, which require infrastructure setup, SLAM does not depend on pre-existing infrastructure. It operates autonomously by creating maps and understanding the surroundings in real-time, making it highly adaptable to changing environments. SLAM relies on data captured by sensors already present in many mobile devices, such as smartphones, and offers a cost-effective solution for accurate localization and mapping without the need for additional hardware or subscription services.

The primary advantage is the achievement of accurate localization, underscoring the crucial role of SLAM in precisely determining a user's position within the environment.
In addition, the real-time performance of SLAM, highlighted in seven studies, empowers real-time global localization and navigation instructions, which are essential for assisting visually impaired users in their immediate environments.
The importance of SLAM in indoor navigation is evident in environments in which GPS signals may be unreliable or absent. 
The robustness and reliability of SLAM, mentioned in seven studies, further emphasize its dependability, even under challenging conditions. 
Another feature acknowledged in the publications is the capacity of SLAM for sensor integration, making it adaptable to various sensory inputs. By effectively utilizing a range of sensors, SLAM shows promise for robust performance even with low-cost, lightweight wearable hardware. 

Moreover, SLAM's capability to map environments underscores its ability to create accurate representations of the surroundings, which is valuable for scene understanding. The integration of semantic information into a map enhances navigation by providing a contextual understanding of the environment, enabling more informed decision making and improved interaction with the surroundings.
Furthermore, several SLAM algorithms can handle large-scale environments. Therefore, users can receive precise information even in expansive spaces, thereby reducing the risk of disorientation and enhancing their safety and confidence while navigating. 

In addition, SLAM enables reliable re-localization, allowing the system to regain accurate positioning, even after a temporary loss of tracking, as evidenced by \cite{zhang2019arcore}. This feature ensures that visually impaired users can reorient themselves quickly, thereby providing a smoother and more confident navigation experience in dynamic environments.
In the context of visually impaired navigation, SLAM's capabilities enable accurate path planning, collision avoidance, and real-time mapping of the environment to perceive surroundings, ultimately facilitating independent navigation of visually impaired individuals in both indoor and outdoor spaces. However, these advantages depend on several factors, including the specific application, choice of sensors, environmental conditions, and algorithmic implementation.
Table \ref{rq2_advantages} categorizes the overall advantages of SLAM and illustrates studies that have harnessed these benefits.

% Table 11. Advantages of SLAM techniques mentioned in the studies included in the SLR
\input{texs/tables/t11_RQ2_SLAM_advantages}

% 
% Limittions
%
\subsubsection{Limitations}
SLAM techniques are essential for many navigation and mapping applications; however, they have several limitations that can affect their effectiveness. One primary limitation is the dependence on geometric features for an accurate operation. Feature extraction is crucial, as it makes the technique vulnerable to environments with unclear or undetectable features. Additionally, the absence of loop-closure detection in some types of SLAM techniques leads to accumulative pose errors in looped trajectories, thereby affecting long-term accuracy. Visual odometry, a core component of SLAM, tends to introduce cumulative errors over time, which can be mitigated by fusing other sensor data such as IMU data. Feature matching capability, such as that used in OpenVSLAM, as described in \cite{yang2022unav}, may become unreliable when there are significant orientation or position discrepancies between two consecutive frames, leading to degraded mapping and localization accuracy.

These limitations have significant effects on assistive technologies based on SLAM for visually impaired navigations. These technologies rely heavily on accurate mapping and localization to help BVI people navigate unfamiliar environments confidently. However, the dependence of SLAM on landmarks, geometric features, and loop closures can result in mapping errors and inaccurate localization. In the absence of distinct features, the system performance is compromised, potentially causing navigation difficulties. Moreover, the accumulation of pose errors over time can lead to inaccurate trajectory estimations, causing disorientation and navigation challenges for visually impaired. To ensure the effectiveness of SLAM-based navigation systems for the visually impaired, addressing these limitations through sensor fusion, improved feature extraction, loop closure mechanisms, and robust error-correction strategies is crucial. Table \ref{rq2_limitations} categorizes the limitations of SLAM adopted in the publications under review.

This table provides insight into the common challenges encountered in these studies. Among these, changing lighting conditions appear frequently, highlighting the significance of lighting variations that can affect the accuracy of the SLAM outputs. The reliance on geometric features, indicating the common need for distinctive visual cues when adopting visual SLAM techniques. The issues of dynamic environments, scalability, and rapid user motion have received considerable attention. Overall, the distribution suggests that lighting, geometric features, dynamic environments, scalability, and rapid motion are prominent and widely acknowledged challenges in SLAM-based navigation for the visually impaired.

% Table 12. Limitations of SLAM techniques mentioned in the studies included in the SLR.
\input{texs/tables/t12_RQ2_SLAM_limitations}

% 
% RQ3
%
\subsection{RQ3. What challenging situations have been addressed?}
Optimal pathfinding, perception of surroundings, and obstacle avoidance are crucial for navigation. Precise localization of a visually impaired user within the environment is essential for these functions to operate effectively. Our surveyed papers addressed the localization problem using different techniques. Some of these studies have explored other navigation-related challenges. We categorized these challenges into two groups: those relevant to environmental complexities and those related to the sensors used to receive environmental data. Dynamic obstacles and crowded spaces constitute the challenges in the first group, whereas challenges related to changing lighting conditions and the rapid motion of users that results in motion blur fall into the second group. As most recent studies have employed cameras to perceive environments, these two challenges have received significant attention. Table \ref{rq3_challenges} lists the studies that investigated these challenges. 

% Table 13. Challenges addressed in reviewed studies using SLAM techniques
\input{texs/tables/t13_RQ3_challenges}

A number of studies under our review used other techniques such as deep learning-based obstacle-avoidance method or the use of other sensors such as ultrasonic to deal with the challenges raised, which are not related to SLAM and are outside the scope of this review. In the following section, we discuss studies that address these challenges by using SLAM techniques.


% 4.3.1 Environmental complexities
%
\subsubsection{Environmental complexities}

%
% Crowded scenarios
%
\textbf{Crowded scenarios}
Navigating crowded environments presents significant challenges for the visually impaired, leading to increased collision risks and difficulties in maintaining personal space. The absence of visual information makes it difficult to measure distance, perceive crowd density, and locate landmarks or places of interest.

Navigation in crowded environments also poses challenges for assistive technologies. For example, in assistive systems that operate based on SLAM, the presence of numerous dynamic elements, such as moving individuals and objects, introduces ambiguity into feature detection and tracking, leading to difficulties in accurately estimating the pose of the user and structure of the environment. The dynamic nature of crowds also hinders loop closure detection, disrupts map consistency, and contributes to drifts. Moreover, the lack of distinct visual landmarks in crowded scenes represents a reliable localization challenge, which potentially reduces the robustness and accuracy of the overall SLAM system. Addressing these challenges requires the development of new approaches to effectively address the complexity of such environments. Some reviewed studies have examined this issue.

\cite{zhang2023research} presented a guide mobile robot engineered for the complexities of navigating different environments while considering dynamic objects and human presence. The robot could handle crowded environments with multiple dynamic objects. To accomplish this, the robot leveraged a spatial risk map, a tool that evaluates potential object-occupied spaces, to chart a path that effectively minimizes disruptions. This study presents experiments in which a robot successfully guided a user through the passage of multiple objects and people.

In another study, \cite{qiu2022egocentric} introduced an egocentric human trajectory forecasting model that was designed for navigation in crowded environments. By leveraging a wearable camera, the model captures detailed surroundings and the user's past trajectory to predict their future. The trajectories obtained using ORB-SLAM3 were used to train the egocentric human trajectory forecasting model, which predicted the wearer's future trajectory based on contextual cues captured by the wearable camera and the wearer's past trajectory.

Additionally, \cite{lu2021assistive} tackled challenges in crowded environments using a combination of SLAM and Ultra-Wideband (UWB) positioning. However, the SLAM algorithm was found to be less effective in environments with dynamic obstacles such as pedestrians. The algorithm would find features of the dynamic obstacles moving along with the robot as the assistive device, and thus it was misled that the robot did not move at all. However, using UWB positioning mitigates this issue.

In \cite{kayukawa2020guiding}, the method addressed crowded environments by recognizing and predicting people's behavior while anticipating the collision risk. The system advises users to adjust their walking speed (on-path mode) or to choose alternative routes (off-path mode). This involves comparing the 3D point cloud map to the real-time LiDAR and IMU sensor data. The system then predicts the future position and velocity of the user in order to avoid collisions.

%
% Dynamic objects
%
\textbf{Dynamic objects}
Several publications have not directly addressed the challenge of crowded environments, and have only focused on dealing with the presence of dynamic objects within the scene. In the system proposed by \cite{ou2022indoor}, dynamic objects can be identified, and average depth information can be provided to the user. When a dynamic object belongs to a predefined class such as a person, it can also be tracked between frames in the SLAM pipeline. The system is capable of identifying and tracking dynamic objects after ego-motion estimation to obtain average depth information. Subsequently, it can estimate the poses and speeds of these tracked dynamic objects and relay this information to the users through acoustic feedback. Depth information helps users maintain social distancing in public indoor environments such as shopping malls.
To address the challenge of dynamic objects, \cite{jin2020combining} proposed a new method called visual simultaneous localization and mapping for moving person tracking (VSLAMMPT). This method was designed to handle dynamic environments in which objects constantly move. The system also uses the expected error reduction with active-semi-supervised learning (EER–ASSL)-based person detection to eliminate noisy samples in dynamic environments. This aids in accurate detection and avoidance of dynamic obstacles.

%
% 4.3.2 Sensor-related
%
\subsubsection{Sensor-related}

\textbf{Changes in lighting condition}
Lighting changes pose a hurdle to visual SLAM systems. Illumination variations alter the visual features, interfere with accurate detection and matching across frames, impact pose estimation, and map-building robustness. SLAM relies on distinctive features for operation; however, lighting changes introduce ambiguities, noise, and errors, which affect the accuracy. Overcoming this challenge requires robust algorithms for dynamic lighting to ensure stable and precise localization and mapping.

The method proposed in \cite{cheng2021hierarchical} tackles the challenge of illumination changes using a deep descriptor network called a Dual Desc, which is designed to be robust against various appearance variations, including illuminance changes. The network uses multimodal images (RGB, Infrared, and Depth) to generate robust attentive global descriptors and local features. These descriptors were used to retrieve coarse candidates of query images, and 2D local features, along with the 3D sparse point cloud, were used for geometric verification to select the optimal results from the retrieved candidates. The authors mentioned that their dataset included images captured at different times of the day, which resulted in illumination changes between the query and database images. Despite these changes, the proposed method achieved satisfactory localization results. 

\cite{zhou2022multi} mentioned that the proposed localization scheme was verified in a typical office building environment with dramatically changing lighting conditions throughout the day; however, it does not provide detailed results or discussion on how changing lighting conditions affect the performance of the system.

The authors of \cite{liu2020indoor} evaluated the influence of lighting conditions on the performance of their novel localization method. The authors captured training images during the day and test images at night and simulated changes in lighting conditions by switching some of the lights off in locations without windows. The results showed that changes in the lighting conditions had a minor impact on the proposed method.

The method proposed in \cite{salihappearance} addressed changes in illumination as a challenge using the COLD and IDOL datasets, which were recorded under different weather and illumination conditions (cloudy, night, and sunny) using different mobile platforms and camera setups. These datasets were used to evaluate the strength of the localization and recognition algorithms with respect to the variations caused by human activities and changes in illumination conditions. The study also mentions the use of Histogram of Oriented Gradients (HOG) for feature extraction, which provides preferable invariant results for lighting or shadowing.

%
% Motion blur
%
\textbf{Motion blur}
Blurred images in visual SLAM can lead to inaccuracies in feature detection and matching, causing issues with pose estimation, map-building, loop closure, and visual odometry. These inaccuracies can also impact depth measurements and map quality. To address this issue, strategies such as using high-frame-rate sensors, incorporating IMUs, and employing motion deblurring techniques can be employed to improve the accuracy of localization and mapping in SLAM systems.
Motion blur can be caused by fast or sudden movements of the user during navigation, which can affect localization performance. \cite{liu2020indoor} studied this challenge and evaluated the robustness of the localization methods. They captured 2316 blurred images on the testing day. The results showed that the proposed method performed poorly in this experiment, indicating that fast motion or sudden changes in user movement could pose a challenge to the system. The reason for this poor performance was that the object detection scores did not exceed the threshold during the experiment.

%
% RQ4
%
\subsection{RQ4. How the proposed solution is expected to enhance mobility and navigation for visually impaired?}
This section discusses how the studies included in our SLR have the potential to improve navigation for BVI people.  These studies focused on diverse attributes, such as accurate pose estimation, semantic mapping, sensor fusion, and algorithmic innovations, to improve BVI navigation quality. Table \ref{rq4_mobility_improvement} presents the categorization of attributes that contribute to enhancing the mobility and navigation of visually impaired individuals. Papers that placed a greater emphasis on these features were referenced within each category.

As expected, most studies adopted SLAM to provide precise localization, which is critical for assistive navigation systems. Precise localization provides accurate information regarding a user's position in the environment in which the user navigates. This accuracy enables the system to offer feedback on obstacles, pathways, and points of interest, thereby allowing the BVI to navigate safely and confidently. Real-time assistance also emerged as a key feature. Providing immediate feedback on the environment enables users to travel efficiently and safely, which leads to increased mobility and independence. 
Semantic mapping, highlighted in eight studies, generates maps beyond geometric data. Such representations contain not only spatial information but also the semantic meanings of objects and features within the environment. This semantic understanding offers a deeper insight into the environment. This contextual awareness is particularly beneficial for enhancing navigation accuracy, as it enables navigation systems to make decisions based on semantic context, improving obstacle avoidance, path planning, and overall navigation efficiency. 

By employing robotic systems such as small robots, smart canes, and sensor-equipped suitcases, seven studies provided guidance, obstacle avoidance capabilities, and increased spatial awareness, thereby effectively providing independent navigation for visually impaired individuals. 
Smartphone-based solutions, also highlighted in seven papers, harness the ubiquitous nature of smartphones that are equipped with cameras and sensors. These solutions offer navigation assistance by using widely available and familiar devices.
As addressed in four papers, both indoor and outdoor navigation capabilities offer a seamless transition between environments, ensuring that users receive consistent support regardless of the scene in which they navigate.
Innovative localization and mapping algorithms, explored in four papers, enhance navigation efficiency and effectiveness through tailored modifications of existing SLAM frameworks or the creation of novel solutions. Ultimately, these advancements have led to an improved overall experience for individuals with visual impairment.
Although these studies focused on different features and attributes, they all aimed to enhance mobility, independence, and overall quality of life for BVI people.

% Table 14. Attributes of SLAM-based navigation systems that contribute to enhancing BVI navigation, along with referenced papers emphasizing
\input{texs/tables/t14_RQ4_mobility_improvement}

==> texs/draft/draft_t11_RQ2_SLAM_advantages.tex <==
% 
%  Table. RQ2. Advantages
% 
\begin{table*}
\footnotesize
% \scriptsize
\centering
\caption{\textbf{Advantages of SLAM techniques mentioned in the studies included in the SLR.}}
\label{rq2_advantages}
\setlength{\tabcolsep}{3pt}
\begin{tabularx}{\textwidth}{p{90pt} X p{75pt}}
\hline
\textbf{Advantages} & \textbf{Description} & \textbf{Reference(s)} \\
\hline
    Accurate localization & Accurate localization is a key advantage of SLAM that ensures the precise determination of a user's position within the environment. & \cite{zhang2017indoor, bai2017cloud, ramesh2018real, slade2021multimodal, hao2022detect, chen2020can, crabb2023lightweight, son2022wearable, hakim2019indoor, chen2020can, weiss2020navigation} \\
    Real-Time performance & SLAM's real-time performance not only ensures immediate and precise localization but also facilitates continuous mapping, providing visually impaired individuals with up-to-date environmental knowledge for safer and more effective navigation. & \cite{zhang2017indoor, kuribayashi2023pathfinder, bai2018virtual, hao2022detect, xu2021multi, son2022wearable, son2022wearable} \\ 
    Robustness and reliability & Robustness and reliability are inherent advantages of SLAM that ensure accurate navigation and mapping, even in challenging scenarios. & \cite{zhang2017indoor, fusco2020indoor, kayukawa2020guiding, hou2022knowledge, plikynas2022indoor, kayukawa20233dmoviemap, eden2018indoor} \\
    Sensor integration & The power of SLAM lies in its sensor integration, which enables the incorporation of diverse sensory information for precise mapping and localization. This enhances BVI individuals’ localization and perception capabilities and empowers them to navigate confidently in unfamiliar settings. & \cite{goswami2023efficient, yang2022unav, zhou2022multi, jin2021wearable, bai2018virtual, yang2022seeway, zhang2019human} \\ 
    Indoor navigation & SLAM offers accurate indoor navigation, which is particularly valuable for BVI individuals in environments in which GPS signals are unreliable or unavailable. This capability ensures that visually impaired users can rely on SLAM technology to maintain precise and dependable orientation and mobility support. & \cite{zhang2017indoor, bai2017cloud, kayukawa2020guiding, zhao2019multi, ramesh2018real, bai2019wearable, lu2021personalized} \\
    Mapping of the environment & SLAM enables the creation of environmental maps, contributing to a better understanding and navigation within different spaces. & \cite{shahani2023methods, zhang2019human} \\
    Large-Scale environments & Several SLAM algorithms can handle large-scale environments effectively. Therefore, users receive precise information even in expansive spaces, thereby reducing the risk of disorientation and enhancing their safety and confidence while navigating. & \cite{endo2017indoor} \\
    Re-localization & SLAM enables reliable re-localization, allowing the system to regain accurate positioning even after a temporary loss of tracking. This feature ensures that BVI users can reorient themselves quickly, thereby providing a smoother and more confident navigation experience in dynamic environments. & \cite{zhang2019arcore} \\
    
\hline
\end{tabularx}
\end{table*}



==> texs/draft/draft_t12_RQ2_SLAM_limitations.tex <==
% 
%  Table. RQ2. Limitations
% 
\begin{table*}[h]
\footnotesize
% \scriptsize
\centering
\caption{Limitations of SLAM techniques mentioned in the studies included in the SLR.}
\label{rq2_limitations}
\setlength{\tabcolsep}{3pt}
\begin{tabularx}{\textwidth}{p{100pt} X p{75pt}}
\hline
\textbf{Limitations} & \textbf{Description} & \textbf{Reference(s)} \\
\hline
    Reliance on geometric features & Accuracy depends heavily on the detection of geometric features, making it susceptible to performance degradation in environments with sparse feature points and distinctive landmarks, potentially affecting the mapping and localization accuracy. & \cite{zhang2017indoor, li2022sensing, hakim2021indoor, zhang2020plane, liu2020indoor} \\
    Loop-closure detection & Without loop-closure detection, a SLAM-based navigation system can accumulate pose errors in revisited areas, leading to inaccurate maps and navigation paths over time. This affects the accuracy and reliability of the system, particularly when a user walks in a looped trajectory. & \cite{zhang2017indoor, rui2021multi} \\
    Cumulative errors and drift & Cumulative errors and drift refer to the gradual build-up of positioning inaccuracies over time. These errors stem from sensor noise, data association issues, and motion estimation inaccuracies, which lead to misalignment with the actual environment and reduced navigation reliability.  & \cite{chen2021wearable, ahmetovic2023sonification, eden2018indoor} \\
    Feature matching & Feature matching involves identifying landmarks in sensor data for mapping and localization. However, issues with large orientation or position differences can reduce the accuracy, causing errors in user motion estimation and affecting the reliability of the navigation system. & \cite{yang2022unav} \\
    Complexity of building map & Building map complexity can lead to computational demands, time-consuming mapping, and potential inaccuracies, particularly in dynamic and complex environments. & \cite{bai2017cloud} \\
    Limitations of sensors & The use of sensors, such as LiDAR and IMU, may have limitations in certain environments, such as areas with low visibility or high levels of interference. In addition, the quality of the sensor data has a significant impact on accuracy. & \cite{kayukawa2020guiding, crabb2023lightweight} \\
      Lighting conditions & Challenging lighting conditions, such as poor lighting, can affect feature detection and tracking, potentially leading to inaccurate localization and mapping. & \cite{chen2020navigation, zhao2019multi, goswami2023efficient, bai2018virtual, rui2021multi, kayukawa20233dmoviemap, chen2020can} \\
    Mapping accuracy & The precision of the constructed map of the environment depends on various factors, such as sensor noise and environmental complexity, which affect the navigation reliability. & \cite{chen2017ccny, hou2022knowledge, xie2022multi} \\
    Dynamic environments & Dynamic objects in the environment can challenge a navigation system's ability to accurately track its own motion and environment, leading to localization and mapping errors. & \cite{rui2021multi, kayukawa20233dmoviemap, lu2021assistive} \\
    Scalability & The challenge of maintaining accurate performance and efficiency as the complexity and size of the environment increases can affect the navigation system's ability to effectively handle larger or more complex spaces. & \cite{rui2021multi, li2022sensing, yang2022seeway, chen2021wearable} \\
    Real-time performance & Although SLAM strives for real-time operation, achieving real-time performance can be challenging. This is dependent on factors such as the complexity of the environment, the computational resources at hand, and the particular SLAM algorithm employed. & \cite{rui2021multi} \\
    Occlusions & Occlusion leads to difficulties in accurately mapping and tracking the environment, which can result in localization errors and a decreased mapping quality. & \cite{li2022sensing} \\
    Rapid motion & The quick movements of users can result in tracking errors, challenges in feature matching, and pose estimation inaccuracies, thereby affecting the ability of the system to maintain accurate localization and mapping. & \cite{xu2021multi, kayukawa20233dmoviemap, li2022sensing, chen2020can} \\
\hline
\end{tabularx}
\end{table*}

==> texs/draft/draft_t14_RQ4_mobility_improvement.tex <==
% 
%  Table. RQ4
% 
\begin{table*}[h]
\footnotesize
% \scriptsize
\centering
\caption{\textbf{Attributes of SLAM-based navigation systems that contribute to enhancing BVI navigation, along with referenced papers emphasizing each feature.}}
\label{rq4_mobility_improvement}
\setlength{\tabcolsep}{3pt}
\begin{tabularx}{\textwidth}{p{90pt} X p{75pt}}
\hline
% Prominent features
% Attribute
\textbf{Features} & \textbf{Description} & \textbf{Reference(s)} \\
\hline
    Precise Localization & Using SLAM algorithms, these solutions accurately estimate the position and orientation of visually impaired users.  Precise localization is essential for visually impaired navigation systems in order to ensure accurate real-time guidance, obstacle avoidance, and spatial awareness, ultimately enhancing independent and safe mobility. & \cite{bai2017cloud, bai2018virtual, slade2021multimodal, chen2020can, liu2020indoor, fusco2020indoor, eden2018indoor, zhang2019human, kayukawa2020guiding, lu2021personalized, xie2022multi, zhou2022multi, yang2022unav} \\ 
    Real-time assistance & This feature ensures that BVI users receive immediate feedback about their environment. Therefore, they can be guided to navigate safely and efficiently, thereby enhancing their overall mobility and independence. & \cite{zhang2017indoor, chen2021wearable, song2023mixture, jin2021wearable, chen2020navigation, hakim2021indoor, xu2021multi, qiu2022egocentric, agrawal2022novel, li2022sensing} \\
    Semantic mapping & Semantic mapping involves creating detailed environmental representations that go beyond geometric data and enables visually impaired users to navigate with a deeper understanding of their surroundings. & \cite{zhao2019multi, chen2020can, liu2020indoor, chen2021wearable, goswami2023efficient} \\
    Hybrid mapping & Hybrid mapping combines short-range vision-based mapping with long-range hybrid mapping to  ensure that visually impaired users receive reliable navigation cues, thereby contributing to their confidence in unfamiliar environments. & \cite{mulky2018autonomous} \\
    Both indoor and outdoor navigation & Systems that serve both indoor and outdoor settings allow users to transition seamlessly between different environments while receiving consistent support. & \cite{bai2017cloud, bai2019wearable, hao2022detect, shahani2023methods} \\
    Innovative algorithms & Innovative algorithms lead to advancements in navigation techniques. These approaches contribute to a more efficient and effective navigation, ultimately improving the overall experience of the visually impaired. & \cite{zhang2017plane, zhang2020plane, jin2021wearable, jin2020combining} \\
    Robotic navigation & These solutions employ robotic systems, such as robots, smart canes, and suitcases, which are equipped with sensors to assist BVI in navigating their environment. & \cite{yun2018design, chen2017ccny, zhang2023research, lu2021assistive, kuribayashi2023pathfinder, rui2021multi, slade2021multimodal} \\ 
    Smartphone based & Equipped with cameras and sensors, smartphones can be considered versatile navigation tools. These solutions offer assistance through devices that are widely available and familiar. & \cite{fusco2020indoor, verma2020indoor, bai2017cloud, ramesh2018real, bai2019wearable, crabb2023lightweight, zhang2019arcore} \\
\hline
\end{tabularx}
\end{table*}

==> texs/draft/t10_RQ1_SLAM_type-20240124.tex <==
% 
%  Table 10. RQ1. What simultaneous localization and mapping (SLAM) approaches are used for visually impaired people navigation?
% 
\begin{table*}[h]
% \footnotesize
\scriptsize
\centering
\caption{\textbf{Localization and mapping approaches used for visually impaired navigation}}
\label{rq1_slam_type}
\setlength{\tabcolsep}{3pt}
\begin{tabularx}{\textwidth}{p{75pt} X p{40pt} p{75pt}}
\hline
\multicolumn{4}{ c }{ \textbf{Widely applicable techniques}} \\
\hline
\textbf{Technique} & \textbf{Description} & \textbf{Sensor type} & \textbf{Reference(s)} \\
\hline
Cartographer & A real-time SLAM software designed to create high-resolution, 2D and 3D maps of indoor and outdoor environments. & LiDAR & \cite{kuribayashi2023pathfinder, zhang2023research, zhou2022multi, kayukawa2020guiding} \\
Hector SLAM & An SLAM framework helps map unknown environments and localizes an agent using a pre-built map. & LiDAR & \cite{hakim2021indoor, yun2018design, hakim2019indoor} \\
Laser-based SLAM & A SLAM technique that is useful in scenarios where accurate mapping and navigation are crucial. & Laser scanner & \cite{albogamy2021sravip, lu2021assistive} \\
LiDAR SLAM & A SLAM technique that uses light detection and ranging  sensors to build a map of an environment and track the agent's pose in that map in real time. & LiDAR &  \cite{slade2021multimodal} \\
Dynamic-SLAM & A system that detects dynamic objects in an environment and understands the motion of the camera. & \textcolor{my_DarkGreen}{Visual} &  \cite{ou2022indoor} \\
LSD-SLAM & A SLAM algorithm designed for monocular cameras is used to create environmental maps and estimate the camera's pose within those maps using only a single camera sensor. & \textcolor{my_DarkGreen}{Visual} &  \cite{endo2017indoor, shahani2023methods} \\
Online SLAM & An SLAM technique that can process sensor data in real time allows the agent to build and update a map of the environment and perform pose estimation while moving. & \textcolor{my_DarkGreen}{Visual} & \cite{agrawal2022novel} \\
OpenVSLAM & An open-source V-SLAM library and framework designed to provide robust and efficient solutions for estimating the camera's pose and creating maps of environments using visual sensor data from cameras. \cite{sumikura2019openvslam} & \textcolor{my_DarkGreen}{Visual} & \cite{yang2022unav, lu2021personalized, chen2020can} \\
ORB-SLAM & A Keyframe- and feature-based monocular SLAM operating in real time in large environments performing camera relocalization from different viewpoints. \cite{mur2015orb} & \textcolor{my_DarkGreen}{Visual} & \cite{xie2022multi, chen2021wearable, rui2021multi} \\
ORB-SLAM2 & An improved version of the original ORB-SLAM builds upon the features and principles of ORB-SLAM while introducing enhancements and optimizations to improve its accuracy, robustness, and overall performance.  \cite{mur2017orb} & \textcolor{my_DarkGreen}{Visual} & \cite{li2022sensing, hou2022knowledge, xu2021multi, weiss2020navigation, chen2020navigation, bai2018virtual, son2022wearable} \\
ORB-SLAM3 & The latest and most advanced version of the ORB-SLAM & \textcolor{my_DarkGreen}{Visual} & \cite{plikynas2022indoor, qiu2022egocentric} \\
Pose-graph SLAM & A SLAM technique that focuses on building a graph to represent the poses of the sensor over time, along with the relationships between those poses. & \textcolor{my_DarkGreen}{Visual} & \cite{zhang2017indoor} \\
RTAB-Map & An RGB-D SLAM approach based on a loop closure detector. & \textcolor{my_DarkGreen}{Visual} & \cite{mulky2018autonomous} \\
Semantic SLAM & An advanced technique that involves not only creating maps and estimating poses but also associating semantic labels with objects or parts of the environment. & \textcolor{my_DarkGreen}{Visual} & \cite{goswami2023efficient, zhao2019multi} \\
Visual SLAM & A technique used to create maps of an environment and simultaneously estimate the camera's pose within that environment using visual sensor data, typically from cameras. & \textcolor{my_DarkGreen}{Visual} & \cite{hao2022detect, kayukawa20233dmoviemap, bai2019wearable, salihappearance, ramesh2018real, lalonde2018localizing, bai2017cloud, crabb2023lightweight, song2023mixture, cheng2021hierarchical, liu2020indoor, chen2017ccny} \\
VI-SLAM & A type of SLAM that uses both visual and inertial sensors to track the motion of an agent and build a map of its environment. & \textcolor{my_DarkGreen}{Visual} & \cite{yang2022seeway} \\
VIO (Visual Inertial Odometry) & A technique that uses both visual and inertial sensors to estimate the pose of an agent in space. & \textcolor{my_DarkGreen}{Visual} & \cite{ahmetovic2023sonification, zhang2019human, fusco2020indoor} \\
\hline
\multicolumn{4}{ c }{ \textbf{ Customized solution}} \\
\hline
DVIO & A depth-enhanced visual-inertial odometry method that performs real-time localization in an architectural floor plan for assistive navigation. & \textcolor{my_DarkGreen}{Visual} & \cite{zhang2021rgb} \\
PAVIO & A method called plane-aided visual-inertial odometry that estimates the 6-DOF (Six degrees of freedom) pose of an agent. & \textcolor{my_DarkGreen}{Visual} & \cite{zhang2017plane, zhang2020plane} \\
RGBD-VIO & A Visual-Inertial Odometry method which tightly couples data from an RGB-D camera and an IMU to estimate device pose for assistive wayfinding. & \textcolor{my_DarkGreen}{Visual} & \cite{jin2021wearable} \\
VSLAMMPT & A SLAM method that eliminates noisy samples in dynamic environments & \textcolor{my_DarkGreen}{Visual} & \cite{jin2020combining} \\
\hline
\multicolumn{4}{ c }{ \textbf{ Spatial tracking frameworks }} \\
\hline
ARCore & A technology that allows ARCore-powered devices to track their position and orientation in the real world. & \textcolor{my_DarkGreen}{Visual} &  \cite{zhang2019arcore} \\
ZED camera’s SLAM & A 6-DoF SLAM technology that allows the ZED camera to track its position and orientation in the real world while also building a 3D map of its environment. & \textcolor{my_DarkGreen}{Visual} & \cite{eden2018indoor} \\
\hline
\end{tabularx}
\end{table*}


==> texs/draft/t11_RQ2_SLAM_advantages20240131.tex <==
% 
%  Table. RQ2. Advantages
% 
\begin{table*}[h]
\footnotesize
% \scriptsize
\centering
\caption{\textbf{Key features of SLAM that benefit visually impaired navigation.}}
\label{rq2_advantages}
\setlength{\tabcolsep}{3pt}
\begin{tabularx}{\textwidth}{p{100pt} X X }
\hline
\textbf{Advantages} & \textbf{Description} & \textbf{Ref.} \\
\hline
    Accurate localization & Accurate localization is a key advantage of SLAM that ensures the precise determination of a user's position within the environment. & \cite{ahmetovic2023sonification, li2022sensing, song2023mixture, hou2022knowledge, xie2022multi, slade2021multimodal, lu2021assistive, hakim2021indoor, zhang2021rgb, jin2020combining, bai2019wearable, zhang2019arcore, bai2018virtual,  zhang2017indoor, zhang2020plane, crabb2023lightweight, son2022wearable, hakim2019indoor, hao2022detect, agrawal2022novel, rui2021multi, ou2022indoor, jin2021wearable, xu2021multi, lu2021personalized, kayukawa2020guiding, chen2020can, fusco2020indoor,zhang2019human, ramesh2018real, lalonde2018localizing, zhang2017plane, chen2017ccny, bai2017cloud, endo2017indoor, yang2022seeway, yun2018design} \\
    Environmental mapping & SLAM enables the creation of environmental maps, contributing to a better understanding and navigation within different spaces. & \cite{li2022sensing, song2023mixture, zhang2023research, yang2022unav, zhou2022multi, xie2022multi, slade2021multimodal, hakim2021indoor, zhang2021rgb, liu2020indoor, jin2020combining, bai2019wearable, zhang2019arcore,  bai2018virtual, zhang2017indoor, albogamy2021sravip, hakim2019indoor, goswami2023efficient, kuribayashi2023pathfinder, agrawal2022novel, rui2021multi, ou2022indoor, xu2021multi, lu2021personalized, chen2020navigation, chen2020can, zhao2019multi, mulky2018autonomous, chen2017ccny, bai2017cloud, endo2017indoor, shahani2023methods, yun2018design} \\
    Map Reuse & & \cite{li2022sensing, zhang2019arcore, bai2018virtual, rui2021multi, lu2021personalized, endo2017indoor} &  \\ 
    Loop closing &  & \cite{li2022sensing, plikynas2022indoor, goswami2023efficient} \\
    Semantic Mapping & & \cite{chen2021wearable, goswami2023efficient, zhao2019multi} \\
    Object localization & & \cite{liu2020indoor, hao2022detect, agrawal2022novel, jin2021wearable} \\
    Dense navigation maps & & \cite{xie2022multi, chen2021wearable, rui2021multi} \\
    Incremental map updating & & \cite{xie2022multi, hakim2021indoor, rui2021multi} \\
    Integration with other technologies & & \cite{xie2022multi, lu2021assistive, liu2020indoor, hakim2019indoor, goswami2023efficient, hao2022detect, rui2021multi, xu2021multi, chen2020navigation, fusco2020indoor} \\
    Integration of sensors & The power of SLAM lies in its sensor integration, which enables the incorporation of diverse sensory information for precise mapping and localization. This enhances BVI individuals’ localization and perception capabilities and empowers them to navigate confidently in unfamiliar settings. & \cite{song2023mixture, albogamy2021sravip, goswami2023efficient, jin2021wearable} \\ 
    Cost-effectiveness and accessibility & & \cite{chen2021wearable, hakim2021indoor, bai2018virtual,  hakim2019indoor, hao2022detect} \\
    Ground-truth trajectory & & \cite{plikynas2022indoor, qiu2022egocentric, bai2018virtual} \\
    Integration with 2D map & & \cite{plikynas2022indoor, zhang2021rgb, zhang2019arcore, zhang2017indoor, crabb2023lightweight, fusco2020indoor} \\
    Dynamic environment handling & & \cite{jin2020combining, ou2022indoor, endo2017indoor} \\
    Semantic information integration & & \cite{son2022wearable}
    Re-localization & SLAM enables reliable re-localization, allowing the system to regain accurate positioning even after a temporary loss of tracking. This feature ensures that BVI users can reorient themselves quickly, thereby providing a smoother and more confident navigation experience in dynamic environments. & \cite{li2022sensing} \\
\hline
\end{tabularx}
\end{table*}



==> texs/draft/t14_RQ4_mobility_improvement-20240130.tex <==
% 
%  Table. RQ4
% 
\begin{table*}[h]
\footnotesize
% \scriptsize
\centering
\caption{\textbf{The overall attributes of SLAM-based navigation systems that contribute to enhancing BVI navigation}}
\label{rq4_mobility_improvement}
\setlength{\tabcolsep}{3pt}
\begin{tabularx}{\textwidth}{p{90pt} X }
\hline
% Prominent features
% Attribute
\textbf{Features} & \textbf{Description} \\
\hline
    Precise Localization & Using SLAM algorithms, the position and orientation of visually impaired users can be accurately estimated.  Precise localization is essential for visually impaired navigation systems in order to ensure accurate real-time guidance, obstacle avoidance, and spatial awareness, ultimately enhancing independent and safe mobility.\\ 
    Real-time assistance & This feature ensures that BVI users receive immediate feedback about their environment. Therefore, they can be guided to navigate safely and efficiently, thereby enhancing their overall mobility and independence. \\
    Semantic mapping & Semantic mapping involves creating detailed environmental representations that go beyond geometric data and enables visually impaired users to navigate with a deeper understanding of their surroundings.\\
    Hybrid mapping & Hybrid mapping combines short-range vision-based mapping with long-range hybrid mapping to  ensure that visually impaired users receive reliable navigation cues, thereby contributing to their confidence in unfamiliar environments. \\
    Both indoor and outdoor navigation & Systems that serve both indoor and outdoor settings allow users to transition seamlessly between different environments while receiving consistent support. \\
    Robotic navigation & Robotic systems, such as robots, smart canes, and suitcases, can be equipped with sensors to assist individuals with visual impairments in navigating their environment. \\ 
    Smartphone based & Equipped with cameras and sensors, smartphones can be considered versatile navigation tools. These solutions offer assistance through devices that are widely available and familiar.  \\
\hline
\end{tabularx}
\end{table*}

==> texs/tables/t_template.tex <==
\begin{table*}
% \footnotesize
 \scriptsize
\centering
\caption{\textbf{}}
\label{tab:}
\setlength{\tabcolsep}{3pt}
\begin{tabularx}{\textwidth}{p{15pt} X X p{60pt} p{15pt} p{40pt}}
\hline
\textbf{Ref.} & \textbf{} & \textbf{} & \textbf{} & \textbf{} & \textbf{} \\
\hline
\cite{ahmetovic2023sonification} &  \\56
\cite{li2022sensing} &  \\57
\cite{song2023mixture} & \\58
\cite{zhang2023research} &  \\59
\cite{yang2022unav} & 60 \\
\cite{zhou2022multi} & \\61
\cite{hou2022knowledge} & \\62
\cite{plikynas2022indoor} &  \\63
\cite{xie2022multi} &  \\64
\cite{qiu2022egocentric} &  \\65
\cite{chen2021wearable} & \\66
\cite{slade2021multimodal} &  \\67
\cite{lu2021assistive} & 68 \\
\cite{hakim2021indoor} &  \\69
\cite{zhang2021rgb} & 70 \\
\cite{cheng2021hierarchical} &  \\71
\cite{liu2020indoor} & 72 \\
\cite{jin2020combining} & \\73
\cite{bai2019wearable} &  \\74
\cite{zhang2019arcore} &  75 \\
\cite{bai2018virtual} & 76 \\
\cite{zhang2017indoor} &  \\77
\cite{zhang2020plane} & 78 \\
\cite{albogamy2021sravip} & \\79
\cite{crabb2023lightweight} &  \\80
\cite{son2022wearable} & 82 \\
\cite{hakim2019indoor} & \\83
\cite{goswami2023efficient} & \\84
\cite{hao2022detect} & \\85
\cite{kuribayashi2023pathfinder} & 87 \\
\cite{agrawal2022novel} & \\88
\cite{rui2021multi} & \\89
\cite{ou2022indoor} & \\90
\cite{jin2021wearable} & \\91
\cite{xu2021multi} & \\92
\cite{lu2021personalized} & \\93
\cite{kayukawa2020guiding} & \\95
\cite{chen2020navigation} & \\96
\cite{chen2020can} & \\97
\cite{fusco2020indoor} & \\98
\cite{zhang2019human} & 99 \\
\cite{zhao2019multi} & \\100
\cite{weiss2020navigation} & \\101
\cite{ramesh2018real} & 102 \\
\cite{eden2018indoor} & 103 \\
\cite{mulky2018autonomous} & 104 \\
\cite{lalonde2018localizing} & \\
\cite{zhang2017plane} & 106 \\
\cite{chen2017ccny} & 107 \\
\cite{bai2017cloud} & \\108
\cite{endo2017indoor} & 109 \\
\cite{yang2022seeway} & \\110
\cite{shahani2023methods} &  \\111
\cite{yun2018design} & \\112
\hline
\end{tabularx}
\end{table*}



\cite{ahmetovic2023sonification} &  \\
\cite{li2022sensing} &  \\
\cite{song2023mixture} & \\
\cite{zhang2023research} &  \\
\cite{yang2022unav} & \\
\cite{zhou2022multi} & \\
\cite{hou2022knowledge} & \\
\cite{plikynas2022indoor} &  \\
\cite{xie2022multi} &  \\
\cite{qiu2022egocentric} &  \\
\cite{chen2021wearable} & \\
\cite{slade2021multimodal} &  \\
\cite{lu2021assistive} &  \\
\cite{hakim2021indoor} &  \\
\cite{zhang2021rgb} &  \\
\cite{cheng2021hierarchical} &  \\
\cite{liu2020indoor} &  \\
\cite{jin2020combining} & \\
\cite{bai2019wearable} &  \\
\cite{zhang2019arcore} &  \\
\cite{bai2018virtual} &  \\
\cite{zhang2017indoor} &  \\
\cite{zhang2020plane} &  \\
\cite{albogamy2021sravip} & \\
\cite{crabb2023lightweight} &  \\
\cite{son2022wearable} &  \\
\cite{hakim2019indoor} & \\
\cite{goswami2023efficient} & \\
\cite{hao2022detect} & \\
\cite{kuribayashi2023pathfinder} & \\
\cite{agrawal2022novel} & \\
\cite{rui2021multi} & \\
\cite{ou2022indoor} & \\
\cite{jin2021wearable} & \\
\cite{xu2021multi} & \\
\cite{lu2021personalized} & \\
\cite{kayukawa2020guiding} & \\
\cite{chen2020navigation} & \\
\cite{chen2020can} & \\
\cite{fusco2020indoor} & \\
\cite{zhang2019human} & \\
\cite{zhao2019multi} & \\
\cite{weiss2020navigation} & \\
\cite{ramesh2018real} & \\
\cite{eden2018indoor} & \\
\cite{mulky2018autonomous} & \\
\cite{lalonde2018localizing} & \\
\cite{zhang2017plane} &  \\
\cite{chen2017ccny} & \\
\cite{bai2017cloud} & \\
\cite{endo2017indoor} & \\
\cite{yang2022seeway} & \\
\cite{shahani2023methods} &  \\
\cite{yun2018design} & \\
